Building A User-Centric and Content-Driven Socialbot

To build Sounding Board, we develop a system architecture that is capable of accommodating dialog strategies that we designed for socialbot conversations. The architecture consists of a multi-dimensional language understanding module for analyzing user utterances, a hierarchical dialog management framework for dialog context tracking and complex dialog control, and a language generation process that realizes the response plan and makes adjustments for speech synthesis. Additionally, we construct a new knowledge base to power the socialbot by collecting social chat content from a variety of sources. An important contribution of the system is the synergy between the knowledge base and the dialog management, i.e., the use of a graph structure to organize the knowledge base that makes dialog control very efficient in bringing related content to the discussion. Using the data collected from Sounding Board during the competition, we carry out in-depth analyses of socialbot conversations and user ratings which provide valuable insights in evaluation methods for socialbots. We additionally investigate a new approach for system evaluation and diagnosis that allows scoring individual dialog segments in the conversation. Finally, observing that socialbots suffer from the issue of shallow conversations about topics associated with unstructured data, we study the problem of enabling extended socialbot conversations grounded on a document. To bring together machine reading and dialog control techniques, a graph-based document representation is proposed, together with methods for automatically constructing the graph. Using the graph-based representation, dialog control can be carried out by retrieving nodes or moving along edges in the graph. To illustrate the usage, a mixed-initiative dialog strategy is designed for socialbot conversations on news articles.

==> chapter_1/_challenges.tex <==
%%%%%%%%%%%%%%%
% Motivate the domain coverage and chaining
%%%%%%%%%%%%%%%
Building a socialbot requires multi-disciplinary expertise,
including data mining, information extraction, natural language processing
(NLP), and etc. 
Here, we discuss the connection between the socialbot and three well-known
research areas, i.e., dialog systems, recommender systems, and knowledge base
(KB) construction.

A socialbot with a goal of providing online information makes it significantly
different from general chit-chat systems and many task-oriented systems.
Therefore, it generates unique research problems for conversational AI.
At the same time, the socialbot still shares many common characteristics with
those dialog systems, allowing us to borrow previous methods and in turn impact
these areas with new insights.
First, the socialbot needs to handle cases when the user wants to know some
specific information such as a trending topic or details about an event.
In this case, the socialbot acts as task-oriented systems, emphasizing success
and efficiency in fulfilling the user requests.
Second, the entertainment nature of the interaction, especially when the user
comes with no specific goals, encourages the socialbot to engage the user in a
conversation for as long as possible, which is a target of general chit-chat
systems as well.
The need of carrying out casual conversations is also aligned with research on
chit-chat systems.

As a conversational gateway to online content, the socialbot sometimes needs to
proactively recommend items to engage users and/or contribute to evolving goals
in the interaction.
Thus, a socialbot can be viewed as a recommender system using conversational
interactions. 
However, challenges of a conversational interface have prevented recommender
systems from the adoption of natural language interactions, leaving the
conversational recommendation as untapped potential.
Therefore, we anticipate that the socialbot can promote the integration of
dialog systems and recommender systems.
Moreover, both research communities can benefit from socialbot research.

Finally, conversational AI systems are supported by a KB, which can be a
collection of entities (e.g., people, product, organization, and places) and
their relationships.
Existing large-scale public KBs are predominately focused on proper
entities (e.g., Freebase \cite{Freebase2008}, DBpedia \cite{DBpedia2015}}) and
common-sense knowledge (e.g., ConceptNet \cite{ConceptNet2004,ConceptNet2017}).
While these types of knowledge are useful for retrieving factual information and
reasoning,
{\it social chat knowledge} also plays an important role in socialbot
conversations.
Examples of social chat knowledge include interesting facts, funny thoughts,
opinions, and recent news.
They are usually novel, amusing, or timely from the perspective of the
conversation partner.
Unfortunately, current KBs have very limited support for supplying social chat
knowledge, and there is no measure for novelty and amusement.
Therefore, it is necessary to construct a KB for socialbots.

{\color{gray}
The following subsections discuss challenges in socialbot research associated
with the dialog system framework, recommendation policy, and KB construction,
respectively.
}
Revise the next three subsections based on the outline.

\subsection{Dialog system framework}
TBD: rewrote this subsection. Describe the open-domain challenge. Motivates the
need of multi-dimensional SLU and hierarchical DM.
Discuss the SLU challenge: ellipsis, implicit speech act, round-based
interaction.
{\color{gray}
Carrying out open-domain conversations is non-trivial and raises challenges such
as coherent domain chaining and smooth domain transitions.
However, since socialbot research is in the early stages, there is limited prior
work to build on.

The first major challenges is the system architecture.
Similar to open-domain dialog systems, the socialbot architecture needs to be
capable of accommodating a variety of domains.
Ideally, the architecture can isolate domain dependencies to avoid combinatorial
explosion in development and maintenance cost as the coverage of domains
increases, while allowing coherent transitions among domains during a
conversation.

Enabling the capability of discussing online content is also challenging.
Furthermore, the discussion needs to be integrated seamlessly with other
types of conversations.
Therefore, it requires joint efforts in spoken language understanding (SLU),
dialog management (DM), and natural language generation (NLG).
}

\subsection{Recommendation policy}
\label{chap1:ssec:recommendation_policy}
TBD: move some of the discussion to future work, and focus on the reward
shaping / analysis part.
{\color{gray}
The dialog policy is arguably the core of a conversational AI system.
It decides the proper system actions based on various factors.
A conversational AI system may have multiple components for handling different
situations.
Since we envision the socialbot sometimes proactively renders information to
users during the conversation, the recommendation policy becomes a very
important part of the dialog policy.
Recommendation algorithms have been extensively studied in the recommender
system literature (see \cite{Ricci2011}).
Nevertheless, recommendation in conversational AI systems brings new challenges.
\begin{itemize}
	\item First, in addition to making the decision on what to recommend, the
		policy needs to consider the timing for making a recommendation since
		greedily recommending items at every turn or frequent recommendation
		confirmation can be annoying. 
	\item Second, to execute a personalized recommendation algorithm, we need to
		come up with a user profile representation.
		The recommendation algorithm learns to align attributes in the user profile
		with those in the knowledge representation.
		{\color{blue}(Mari's comment: classical recommender systems also build user
		profiles incrementally. Needs to be more clear about the difference.)}
		Unlike classical recommender systems, the user profile is now incrementally
		constructed through conversational interaction.
		It can still be bootstrapped using other contextual information when
		available.
	\item Third, data-driven methods for learning the recommendation policy
		{\color{blue}are attractive?}, but we need to have an initial system to
		collect data and
		extract supervision signals.
		The initial system can use a manually-designed recommendation policy,
		and
		% the recommendation policy can be either manually designed based
		% on domain expertise or learned using data-driven methods.
		% The former is necessary to develop or bootstrap an initial system.
		% Meanwhile, data-driven methods are attractive considering the amount of data
		% can be collected once the initial system is deployed.
		% For developing data-driven models, supervision signals are needed.
		numerical feedbacks can be collected 
		% for conversational AI systems
		by asking for a conversation-level rating after the user completes a
		session.
		However, a conversation session can involve multiple transactions (e.g.,
		topics in the socialbot conversation) and each transaction consists of
		multiple recommendation actions.
		Therefore, it is desirable to develop methods to automatically derive
		scores for individual transactions and recommendation actions using the
		conversation-level ratings.
		Another type of feedback commonly used in classical recommender
		systems is the user behavior feedback such as the click through rate and the
		conversion rate of purchasing a product.
		For socialbots, sources of feedback include the sentiment and the intent
		reflected in user utterances.
		To extract these signals, we need to develop NLP tools such as sentiment
		and intent classifiers.
\end{itemize}
}


\subsection{KB construction}
\label{chap1:ssec:knowledge}
{\color{gray}
A KB can be constructed either manually or automatically.
Manually curated KBs usually rely on a closed group of experts (e.g.,
Cyc/OpenCyc \cite{CYC1995}, WordNet \cite{WordNet1995}) or an open group of
volunteers (e.g., Freebase \cite{Freebase2008}, Wikidata \cite{Wikidata2014}).
Automatic approaches can use semi-structured text (e.g. YAGO
\cite{YAGO2007,YAGO2015}, DBpedia \cite{DBpedia2015}) or unstructured text
(e.g., Knowledge Vault \cite{KnowledgeVault2014}, NELL \cite{NELL2015}, ReVerb
\cite{Reverb2011}).
The choice of KB construction paradigms needs to take into account their
accuracy, coverage, and scalability.

A socialbot needs to have three types of knowledge:
its own backstory (e.g., name, age, hobbies),
factual knowledge (e.g., definition of an entity), 
and social chat knowledge (e.g., recent news, interesting facts, amusing
content).
For backstory knowledge, manual curation is possible and probably preferred.
Existing KBs can provide good support for factual knowledge at scale.
The least studied problem in the literature is the acquisition of social chat
knowledge, as well as the integration of it with other knowledge.
{\color{orange}TBD: what about bot opinions?}

Considering scalability, automatic methods are preferred for acquiring
social chat knowledge.
While Wikipedia is a popular hub for harvesting factual knowledge,
social media platforms such as Twitter and Reddit may be potential sources of
social chat knowledge due the nature of discussions posted there.
Additionally, the KB construction process can exploit social tags and topics
compiled by social media users. 
Nevertheless, using online discussions brings challenges due to the huge
diversity of user generated content.

\begin{itemize}
	\item First, unlike Wikipedia where the quality of the knowledge is generally
		good, online discussions inevitably contain useless, boring, inappropriate, and
		even wrong information.
		A family-friendly socialbot should avoid mentioning content about sex,
		violence, racism, hate speech, and etc.
		Therefore, the KB needs to be extremely careful about the social
		appropriateness of the content.
		Also, one can to measure the ``quality'' of the content from different
		aspects such as informativeness, authority, popularity, novelty, and
		etc.
		Using multiple measures may be useful for different types of content and/orr
		for serving different types of users.
	\item Second, while historical facts are generally static, information about
		places, organizations, and living person often changes.
		{\color{orange}(mention news event, changing opinions?)}
		Dealing with the evolving knowledge remains an unsolved problem in KB
		research and should be taken into account when extracting social chat
		knowledge.
	\item Finally, in order to carry out a deep and engaging discussion on some
		news article, a generic summarization strategy is not enough.
		Instead, we need to identify interesting discussion points from the document
		and represent relations between the points associated with questions that a
		user might ask.
\end{itemize}
}



==> chapter_1/_trash.tex <==
Historically, in the literature, chatbots have adopted very different approaches
from task-oriented systems including both system frameworks and evaluation
methods, perhaps because of the differences in the user's goal and application
scenarios.
On the other hand, there are a variety of commercial intelligent personal
assistants in the market, such as Amazon Alexa, Apple Siri, Google Assistant,
and Microsoft Cortana, which have demonstrated the importance and usability of
combining task-oriented and casual interactions for providing comprehensive user
experience in their daily life.
% Therefore, a question emerges: can approaches in task-oriented systems applied
% to developing a chatbot whose goal is not accomplishing a specific and
% well-defined task?

Now, there are a variety of commercial intelligent personal assistants in the
market, such as Amazon Alexa, Apple Siri, Google Assistant, and Microsoft
Cortana.
As it can be observed from these systems, both task competition and
entertainment are important to provide comprehensive user experiences in their
daily life.


% Thus, next-generation conversational AI systems are expected to be capable of
% both casual interactions and task-oriented conversations, with a blurred
% boundary between the task-oriented systems and chatbots.

% In this scenario, the system needs to handle user goals that are specific and
% explicitly informed (e.g., booking a restaurant), as well as less specific and
% usually implicit user goals (e.g., browsing information,
% entertainment).\hfang{and KB}
% In the latter case, it is desirable to proactively probe and elicit user goals
% and preferences during the conversation.

% As it can be observed from existing commercial intelligent personal assistants
% (e.g., Amazon Alexa, Apple Siri, Google Assistant, Microsoft Cortana),
% both task competition and entertainment are important to provide comprehensive
% user experiences.

Exploratory conversation.

% Now, there are a variety of commercial intelligent personal assistants in the
% market, such as Amazon Alexa, Apple Siri, Google Assistant, and Microsoft
% Cortana.
% , these personal assistants have blurred the boundary of
% task-oriented systems and chatbots, since task competition and entertainment are
% both important to provide comprehensive user experiences.
% \hfang{discuss the knowledge base issue, and the trend to move towards larger
% KB.}

Next-generation conversational AI systems are expected to be capable of social
interaction while handling complex goal-oriented conversations.
In this scenario, the system needs to handle user goals that are specific and
explicitly informed (e.g., booking a restaurant), as well as less specific and
usually implicit user goals (e.g., browsing information,
entertainment).\hfang{and KB}
In the latter case, it is desirable to proactively probe and elicit user goals
and preferences during the conversation.

The {\bf socialbot}, in particular, is an emerging research area in
conversational AI that needs to deal with implicit user goals.
It has a wide range of applications including education, companionship, gaming,
and information acquisition.
While there are different types of socialbots, in this thesis, we focus on the
socialbot that challenges university teams in the Amazon Alexa Prize
\cite{AlexaPrize2017}.


% The Alexa Prize provides a new and unique platform for researchers to build and
% test socialbots by allowing the systems to interact with millions of real users
% through Alexa-enabled devices.
% 
% requires different dialog strategies,
% and large KB, and usntructured data.
% Impacts the technologies and approaches. 
% Furthermore, evaluation.
% ``Casual social conversation presents a problem where dialogue success does not primarily depend on
% the acquisition of information by one or more participants, but also on ‘buy-in’
% or engagement in the activity of talking itself, in addition to the construction and
% maintenance of a social bond.''~\cite{Gilmartin2019IWSDS}.


The general framework described in this thesis is used to develop our socialbot
that won the inaugural Alexa Prize in 2017 \cite{Fang2018NAACL}.

% A new system framework is also needed for handling a wide variety of real users
% in the Alexa Prize setup.
% In this work, we take the general pipeline approach in task-oriented dialog
% systems to develop the socialbot whose goal is not accomplishing a specific and
% well-defined task.
% The system developed in this thesis won the inaugural Alexa Prize in
% 2017~\cite{Fang2018NAACL}.


The work presented in this thesis covers a complete socialbot system for
discussing popular topics and recent events, as challenged by the recent Alexa
Prize \cite{AlexaPrize2017}.

The general framework described in this thesis is used to develop our socialbot
that won the inaugural Alexa Prize in 2017 \cite{Fang2018NAACL}.


A new system framework is also needed for handling a wide variety of real users
in the Alexa Prize setup.

% For task-oriented dialog systems, users usually have a specific goal when
% initiating the conversation, and they normally end the conversation when the
% system succeeds or fails in completing the task. 
% Therefore, recent research efforts are mostly made on improving language
% understanding and dialog management for task completion with higher accuracy and
% efficiency.
% On the other hand, efforts on non-task-oriented chatbots are made to simulate
% human language for coherent conversations, generation.
% For the Alexa Prize socialbot studied in this thesis, the system needs to handle
% evolving user goals which can be either explicit or implicit.

We approaches the problem of discussing popular topics and recent news by
developing the bot as a conversational gateway to online content.
To address the issue of evolving and implicit user goals, the bot proactively
probes and elicits user goals during the conversation. 
The major contributions of this work are summarized below.


\begin{itemize}
	\item Dialog strategies
	\item content-driven, user-centric -- mixed-initiative strategies
	\item apply task-oriented framework to chatbots
	\item hiearahical DM framework for dialog control
	\item large KB to support content
	\item unstructured data to support content
	\item evaluation
\end{itemize}

\begin{comment}
\begin{itemize}
	\item Chapter 2: Background
		\begin{itemize}
			\item dialog system applications: chit-chat,
				task-oriented, problem-solving, etc. new: Alexa Prize socialbot.
			\item SLU: grammar-based and model-based. problem: multiple intents,
				ellipsis (requires context), informal grammar, implicit speech act.
				Engagement analysis.
			\item DM frameworks: CMU RavenClaw (plan-based). Neural-based.
				Require more flexible framework.
			\item NLG framework: review recent neural-based approach.
			\item Dialog system evaluation and diagnosis. PARADISE and recent Alexa
				Prize papers.
			\item KB construction methods.
			\item (Optional) dialog datasets (with and without KB).
		\end{itemize}
	\item Chapter 3: Sounding Board system
		\begin{itemize}
			\item dialog system architecture
			\item KB construction
			\item post-competition development (?)
		\end{itemize}
	\item Chapter 4: Analysis and multi-level rewards.
	\item Chapter 5: KG for deeper discussion about a news article.  Dialog
		strategies to discuss news articles.
		Updates in the framework (here or Chapter 3?).
	\item Chapter 6: Conclusion and Future directions.
\end{itemize}
\end{comment}


==> chapter_2/_background.tex <==
Researchers in AI have long been interested in the challenge of developing a
system that can have a coherent conversation with humans: early systems include
Parry \cite{Colby1975AI}, Eliza \cite{Weizenbaum1996Comm}, and Alice
\cite{Wallace2009ALICE}.
The Loebner Prize\footnote{\url{http://aisb.org.uk/events/loebner-prize}} is a
Turing test for conversational AI that has challenged researchers since 1990.
Recent work has addressed tasks where passing the Turing test is not a concern.
Goal-oriented conversational systems facilitate natural user interaction with devices via text and spoken language. These AI assistants typically focus on short interactions, as in commercial products such as Amazon Alexa, Microsoft
Cortana,  Google Assistant, and Apple Siri. General conversational systems,
called chatbots, have constrained social interaction capabilities but have
difficulty
generating conversations with long-term coherence
\cite{serban2017hierarchical,sato2017modeling,shao2017generating,tian2017make,Ghazvininejad2018AAAI}.

The Alexa Prize sets forth a new challenge: creating a system that can hold a
coherent and engaging conversation on current events and popular topics such as sports,
politics, entertainment, fashion and technology
\cite{AlexaPrize2017}.

\begin{itemize}
	\item Dialog systems: goal-oriented SDS, chit-chat bots, end-to-end models. 
	\item Recommendation systems (critique-based).
	\item Knowledge graph construction.
	\item Discussion: 1) gap between commercial and research systems; 2) gap
		between dialog systems and recommendation systems; 3) knowledge graph for
		socialbots.
\end{itemize}

\section{Dialog Systems}
Applications and history.

\section{SLU}
Frame-based semantics dates back to.
For dialogs, SLU.
mental states.

\section{DM frameworks and Discourse Theories}

\section{Knowledge Graph}
NELL \cite{NELL2015}
OpenIE \cite{Etzioni2011IJCAI}

\section{Dialog System Evaluation}


==> chapter_2/_framework.tex <==
\begin{figure}[t]
	\centering
	TBD
	\caption{General framework.}
	\label{chap1:fig:general_framework}
\end{figure}

Hosted on Alexa-enabled devices in the U.S., Alexa Prize socialbots can interact
with users by voice using speech interface provided by the Alexa Prize platform. 
The Alexa Prize platform routes user's invocation utterance 
``{\it let's chat}'' or its variants to a randomly selected competing socialbot.
The user can terminate the conversation at any time using an explicit {\it stop}
command.
Afterwards, users can rate the system by responding to the question: 
``{\it On a scale of one to five, how much would you like to speak to this
socialbot again?}''

Several socialbot frameworks are developed in the inaugural Alexa Prize
\cite{CMUMagnus2017,CMURubyStar2017,CTUAlquist2017,EmUEmersonbot2017,HWUAlana2017,PrincetonPixie2017,RPIWiseMacaw2017,SNUChattyChat2017,UCBEigen2017,UCSCSlugbot2017,UEdinburghEdina2017,UMontrealMILA2017,UTrentoRovingMind2017,UWSoundingBoard2017}.
This thesis discusses and extends the framework of the 2017 winning
system -- Sounding Board \cite{Fang2018NAACL}.
As illustrated in Fig.\,\ref{chap1:fig:general_framework}, it mainly consists of a
modularized conversation engine and a social chat knowledge graph. 


\subsection{Modularized conversation engine}
The conversation engine uses a centralized logic controller.
The controller produces a system response for the incoming user utterance by
sequentially communicating with three typical dialog system modules, i.e., SLU,
DM, and NLG.
\begin{itemize}
	\item The SLU module offers the capability of understanding user utterances
		from multiple dimensions with different granularities.
	\item The DM module establishes the communication between the conversation
		engine and the social chat knowledge graph. 
		It is equipped with a collection of dialog policies for deciding system
		actions under different scenarios.
	\item The NLG module provides support for rendering an abstract representation
		of the system response in natural language.
		It also supports fine tuning the system response, e.g., grammar correction,
		prosody adjustment, and profanity filtering.
\end{itemize}

Each module registers its capabilities and other information in the controller.
A motivation of using a centralized controller in this way is to maximize the
independence between these three major modules for easier development and
maintenance, while allowing a certain level of awareness and communication
between each other through the centralized controller.

When receiving an incoming user utterance, the controller first collects
necessary information with the help of the SLU module.
The SLU module may use some context information about the DM module maintained
in the controller.
Then, the controller sends the collected information to the DM module to make a
plan about the system response at the speech act level.
Apparently, the DM module needs to know the available speech acts registered by
the NLG module in the controller.
Finally, the controller uses the NLG module to realize the response in the form of
natural language.


\subsection{Social chat knowledge graph}

\begin{figure}[t]
	\centering
	TBD
	\caption{Social chat knowledge graph.}
	\label{chap1:fig:knowledge_graph}
\end{figure}

We use a graph structure to describe the KB storing the social chat knowledge.
Each node in the graph holds a collection of information that characterizes a
entity, a general concept, or a content snippet.
The directed edges represent asymmetric relationships between two nodes.
An example of the knowledge graph is illustrated in
Fig.\,\ref{chap1:fig:knowledge_graph}.

Nodes in the graph have different properties.
One important property is the node type.
Traditional node types are mostly entities (e.g., person, organization, places)
and general concepts.
We introduce a new general node type -- social chat content.
These nodes hold complete content snippets that are generally well suited for
social chat conversations. 
Examples of such content snippets include facts, thoughts, jokes, and news
titles.

Nodes in the knowledge graph can have a variety of relationships, which are
usually discovered using some information extraction algorithm.
Due to the introduction of social chat content nodes, we also create a new pair
of relationships, i.e., \texttt{Mentions} and \texttt{MentionedIn}.
For example, a news title may mentions a movie director, who may be mentioned in
some interesting trivia.
In this way, the social chat content nodes become connected through some
intermediate nodes that represent a entity or a general concept.


==> chapter_2/_system_arch.tex <==
While dialog system architectures vary depending on their applications and
evolve as the speech and language processing technology advances, there are two
typical architectures that are commonly used in recent literature and adopted by
existing Alexa Prize socialbots.
The conventional modularized system.
The neural end-to-end.

\subsection{Speech processing and synthesis}
Dialog systems can interact with users via different modalities, including
speech, text, vision, etc.
In this thesis, we focus on the speech-based dialog systems, although we \dots

{\bf ASR}:
The ASR module transcribes raw audio signals of user utterances to textual form
output.
A common output format is the N-best list, which consists of $N$ most likely
hypotheses of the user utterance associated with their confidence scores.
A richer output format includes the confidence scores for individual words,
which are calculated from the word lattice or confusion
network~\cite{Mangu2000findingconsensus}.

{\bf TTS}:
The TTS module converts system utterance from text to voice signals.
Fine control of the synthesis can be achieved using the Speech Sythnesis Markup
Language (SSML) which can specify prosody, speaking rate,
etc.\footnote{\url{https://www.w3.org/TR/2004/REC-speech-synthesis-20040907}}

Raw audio signals are not accessible to Alexa Prize socialbots for reasons like
privacy.
Instead, Alexa Prize socialbots rely on Amazon's ASR API and receive the N-best list
associated with confidence scores at both utterance and word levels.
Similarly, Amazon's TTS API is used to synthesize Alexa's voices.


\subsection{Modularized architecture}
A representative architecture for modularized dialog systems is illustrated in
Fig.\,\ref{fig:modularized_arch}.
There are four typical components:
a spoken language understanding (SLU) module, a dialog management (DM) module, a
natural language generation (NLG) module, and a back-end knowledge base (KB).
{\color{red}(Several Alexa Prize socialbots follow this \dots?)}

\begin{figure}[t]
	\centering
	TBD
	\caption{A modularized dialog system architecture.}
	\label{fig:modularized_arch}
\end{figure}

{\bf SLU}:
Grammar-based.
Statistical, in the form of intent-slot.


{\bf DM}: 
state-based DM,
plan-based DM.

{\bf NLG}:
template-based.




\subsection{}
% The output, which we call {\bf meaning representation} here, provides necessary
% information for the socialbot to come up with an appropriate response.
% There is no consensus among socialbots on the specifications of the meaning
% representation and corresponding analyses. 
% Several socialbots carry out intent analysis, entity analysis,
% and sentiment analysis(?), although they define and organize corresponding
% meaning representation attributes differently.

% A richer meaning representation is desired to facilitate the dialog management
% and response generation processes.
% In practice, the socialbot needs to strike a balance between the complexity of
% the meaning representation and the available .

% In practice, the meaning representations are designed quite differently.
% the corresponding analyses are organized and implemented quite differently.
% While we try our best to minimize the discrepancy, we may not use the exact same
% terminologies and organizations as in the original papers to make the comparison
% between socialbots easier.
% For example, Chen et al.\ describe the intent classifier as part of the dialog
% management instead of the language understanding process
% \cite{UCDavisGunrock2018}.
% Here, we identify several analyses that are commonly used by existing
% socialbots.

% {\bf Intent Analysis}:
% One way to categorize user utterances is based on the user's intention reflected
% in the utterance.
% For example, the utterance ``{\it can we do something else}'' indicates the
% intent of changing the topic;
% the utterance ``{\it what do you think}'' is opinion seeking.
% Several papers explicitly mention the use of an intent analysis component and
% develop their own set of intents, to name a few:
% \cite{CTUAlquist2017,CTUAlquist2018,HWUAlana2017,HWUAlana2018,CMURubyStar2017,UCDavisGunrock2018}.
% The RubyStar defined 42 common intents by labeling 10K user utterances
% \cite{CMURubyStar2016}.
% The Gunrock \cite{UCDavisGunrock2018} mentioned, but no exact number. 



% Sometimes ``dialog act'' which is rooted from the speech act theory \cite{} is used
% interchangeably with ``intent''.
% 
% Most socialbots are equipped with an intent analysis module, {\color{red} as
% illustrated in}.
% In the task-oriented dialog systems, \dots is traditionally approached as
% identification of the intent and detection of its arguments from a user
% utterance \cite{TurSLUChap3}.
% In a task-oriented and domain-specific SLU, the set of intents and slots is
% usually pre-defined.
% 
% \cite{UTrentoRovingMind2017}: DiaML ISO standard for dialog act annotation.

% Nevertheless, there are three factors that complicate the intent analysis.
% First, the intent inventories differ since the conversation strategies and the
% required granularity of intent for socialbots are different.
% Some socialbots only uses the high-level dialog acts.
% For example, 
% The Sounding Board described in this thesis uses an inventory of 17 intents,
% categorized into five broad groups -- menu commands, chat commands, dialog
% control commands, other commands, and non-commands.
% core act.

Second, an unsegmented utterance may reflect multiple intents, e.g., 
``{\it I don't like sports let's talk about something else}'' indicates both
dislike intent and topic changing intent.
To address this issue, some socialbots carry out segmentation and allow multiple
intents in one utterance.
The Sounding Board system in this thesis uses the heuristic that command, and
carry out fine-grained analysis in parallel.
Roving Mind
Third, context matters.
Sentence completion. Separate context-dependent process.



``yes'' and ``no'' answers are treated as separate intents in some socialbots,
whereas treated as a general ``answer'' intent in others, with the qualifier
represented in other attributes.

Some socialbots include a topic switch intent?


Dialog acts.
Single intent vs.\ multiple intents.
Topic switch intent.
Some may include sentiment as one intent category.

{\bf Contextual Processing}



either shared across multiple modules, or module dependent.
Canonical language understanding.
Utterance representation.

University of Montreal's system \cite{UMontrealMILA2017}: NER

Some teams do not describe an explicit/separate language understanding module,
although the system still is equipped with a language understanding components,
e.g., NER in \cite{UMontrealMILA2017}, intent in \cite{RPIWiseMacaw2017}.
We omit discussions on these systems since \dots.

\begin{table}
	\centering
	\begin{tabular}{l|l}
		\hline\hline
		\hline
		Alana \cite{HWUAlana2017}
		& sentence completion / contextual preprocessor (context-dependent), indirect question analysis,
		intent detection, POS, NER, anaphora resolution. \\
		Alana v2 \cite{HWUAlana2018}
		& Truecaser, contextual preprocessor (context-dependent), POS, intent, NER,
		sentment, entity linking, topic/domain classifier, anaphora resolution, \\
		%
		Alquist \cite{CTUAlquist2017} 
		& sentiment analysis, NER, Sentence Splitting, 
		TrueCase, POS tagging, tokenization, dependency parsing, lemmatisation,
		entity linking (Microsoft Concept Graph; YodaQA/Freebase ID); intent
		detection;
		topic-specific analysis (i.e., dialog-agent NLU phase) for context updates
		and entity linking (it was called entity recognition) for key-phrases \\
		% 
		Alquist v2 \cite{CTUAlquist2018} & intent, NER, dialog act detection (but only the feature vector
		is used for DM), entity sentiment (Twitter
		sentiment about this entity), \\
		%
		Edina \cite{UEdinburghEdina2017} & tokenization, coref, ner, user modeling,
		topic switch intent detection, likes and dislikes, \\
		%
		Eigen \cite{UCBEigen2017}
		& none \\
		Emersonbot \cite{EmUEmersonbot2017} 
		& intent, entity \\
		%
		Pixie \cite{PrincetonPixie2017}
		& sentiment, POS, dependency, NER, coref, (no intent) \\
		% 
		Roving Mind \cite{UTrentoRovingMind2017}
		& dialog acts + qualifiers (function unit) / intent, entity, truecaser, NER, sentence
		split,  entity linking \\
		% 
		RubyStar \cite{CMURubyStar2017}
		& 42 intents, topic/domain, entity disambiguation/linking, \\
		% 
		Magnus \cite{CMUMagnus2017}
		& intent, coref, entity?, sentiment, topic switch detection \\
		% 
		SlugBot \cite{UCSCSlugbot2017} & 
		dependency, POS, sentiment, coref, entity recog, topic classifier \\
		SlugBot v2 \cite{USCSSlugbot2018} & 33 intents, entity disambiguation, topic classifier \\
		%
		MILA \cite{UMontrealMILA2017} & NER; (none) \\
		% 
		BYU-EVE \cite{BYUEve2018} 
		& topic detection, entity/keyword, offensive speech, intent (multiple
		intents) \\ 
		%
		Fantom \cite{} 
		& NER, coref, lemma, sentiment, POS, LDA, topic clf, yes-no-q clf. \\
		% 
		Gunrock \cite{}
		& NP, topic, sentiment, profanity, NER, coref, entity linking, DA, intent \\
		%
		IrisBot \cite{}
		& NER + linking, coref, topic, 11 intents \\
		% 
		Tartan \cite{}
		& intent, topic, sentiment, NER, coref/anaphora, 37 major concepts \\
		%
		Sounding Board \cite{UWSoundingBoard2017} & NER, sentiment\\
		% 
		Seoul National Univ. \cite{SNUChattyChat2017}
		& intent, keyword/entity recog, casual vs. chat \\
		RPI \cite{RPIWiseMacaw2017}
		& intent; none \\
		\hline\hline
	\end{tabular}
	\caption{Language understanding analyses for user utterances.}
	\label{chap2:tab:nlu}
\end{table}
% & Intent & NER & Entity Linking & Coreference & Anaphora & Sentiment & Topic \\
% \checkmark 

Question analysis in Sounding Board.
Embedding in Tartan.



% Script-based methods require developers to write the logics for assembling
% appropriate responses given the context.
% taking into account possible conversations a user might have with the bot.
% One type of script-based methods uses pre-defined rules to code the logics.
% While rules can take into account various of conditions, here we specifically
% refer to rules that do not rely on the rich language understanding described in
% \S\ref{chap2:ssec:nlu} and instead perform pattern matching on the surface form
% of user utterances.
% The ELIZA~\cite{Weizenbaum1966Comm} is a well-known rule-based chatbot.
% It is included in the MILA~\cite{UMontrealMILA2017} and the
% Slugbot~\cite{UCSCSlugbot2017,UCSCSlugbot2018} to handle personal questions.


% \cite{UMontrealMILA2017}: learned ranker/retrieval model (neural, logit)
% Edina: not learned scoring function
% Tartan: hmm, hard to classify
% Eve: not sure how to describe, but indeed there is retrieval
% Fantom: ahh, crowdsourcing, graph-search, like retrieval, grid-search to
% deterimnet he weights,
% RubyStar: retrieve Twitter
% Alana: Reddit without rewritten


% Two typical architectures are used by Alexa Prize socialbots competed in 2017
% and 2018, as illustrated in Fig.\,\ref{chap2:fig:architectures}.
% Both architectures uses a collection of response generation modules.
% The ?? architecture uses a module selector before invoking the response generation
% module to construct the bot response \cite{}.
% The post-?? architecture executes all available response generation modules and
% uses a response ranker to select one response \cite{} or combing multiple best
% responses \cite{} as the bot response.
% Tartan uses both.
% It is difficult to find a universal response strategy that can engage users on
% discussing popular topics for a long time.
% Considering the wide range of topics and user requests anticipated by Alexa
% Prize socialbots, competing systems usually adopt a modularized design, where
% each component implements a specific response generation method.


==> chapter_2/_trash.tex <==
Another type of conversational AI systems, i.e., {\bf task-oriented dialog
systems}, was used primarily in applications with specific tasks.
% puts more emphasizes on accomplishing specific tasks.
One of the earliest commercial task-oriented systems is the AT\&T How May I Help
You system deployed for routing customers calls to the correct
destination~\cite{Gorin1997SpeechComm}.
DARPA's initiatives on the Airline Travel Information
System~\cite{Price1990ATIS} and the Communicator project~\cite{Walker2002ICSLP}
also contributed to the advance of this research area.

% Now, there are a variety of commercial {\bf intelligent personal assistants} in
% the market, such as Amazon Alexa, Apple Siri, Google Assistant, and Microsoft
% Cortana.
% To some extent, these personal assistants have blurred the boundary of
% task-oriented systems and chatbots, since task completion and entertainment are
% both important to provide comprehensive user experiences.

The {\bf socialbot} is an emerging research area in conversational AI that needs
to deal with implicit user goals.
It has a wide range of applications including education, companionship, gaming,
and information acquisition.
While there are different types of socialbots, in this thesis, we focus on the
socialbot that challenges university teams in the Amazon Alexa Prize~\cite{AlexaPrize2017}.

Traditionally, task-oriented systems are built for limited domains described by
an underlying ontology, which is essentially a structured representation of the
database of entities that the dialog system can talk about.
Such systems typically have access to a database which contains all the
information about the particular domain.
The size of the domain can thus be defined in terms of the size of the
underlying database, which in turn can be described in terms of the number of
entities, attributes, and values.

The semantic web is an effort to organize a large amount of information
available on the Internet into a structure that can be more easily processed by
a machine designed to perform reasoning about this data.
Large-scale knowledge base are 


==> chapter_3/_alexaprize.tex <==
With the goal of advancing the research in conversational AI, Amazon announced
the Alexa Prize on September 26, 2016 and set forth a new challenge for the
research community: creating a {\bf socialbot} system that can hold a coherent
and engaging conversation on current events and popular topics such as sports,
politics, entertainment, fashion and technology \cite{AlexaPrize2017}.
With the Alexa Prize infrastructure supported by the competition organizers,
university teams participating the competition can release their
socialbots to a large user base consisting of millions of Alexa users.
The infrastructure also allows competing teams to access the N-best hypotheses
of user utterances from Alexa's speech recognition output, which are not
available to public Alexa skill developers.

{\bf Competition Setup}:
The socialbot systems interact with users through voice using the Alexa's speech
interface.
The conversation is always initiated by the user with the invocation phrase 
{\it ``let's chat''} or its variants, and the user is routed to a randomly
selected competing socialbot system. 
Currently, Alexa devices only support round-based interactions, i.e., the
socialbot system needs to wait for a user turn before proceeding to its next
turn.
The user can terminate the conversation at any time using an explicit 
{\it ``stop''} command.
Afterwards, the user can rate the system by responding to the question: 
{\it ``On a scale of one to five, how much would you like to speak to this
socialbot again?''}
To reduce bias, the competing socialbot systems are not allowed to reveal the
team's identity during the conversation.

{\bf Finals Evaluation}:
In the 2017 Alexa Prize competition, three finalist socialbot systems (the Alana
\cite{HWUAlana2017}, the Alquist \cite{CTUAlquist2017}, and our Sounding Board
\cite{UWSoundingBoard2017}) are evaluated by a panel of three independent
judges.
The judges listen to the live conversation carried out by a user and a finalist
socialbot, and the conversation is rated by each judge on a scale of 1 to 5
(higher is better).
The user is instructed to keep the conversation going until two of three judges
have pressed the stop button.
Each finalist socialbot carries out two conversations with the same user, and
there are in total three users participating the finals evaluation. 
Our Sounding Board won the finals with an average score of 3.17 and an average
conversation duration of 10:22.

{\bf Discussion}:
The Alexa Prize socialbot is a novel application of conversational AI.
Particularly, the goal of discussing popular topics and recent events makes it
significantly different from traditional task-oriented and chit-chat systems.
Because of the novelty, there is no prior dialog system developed for this
application, nor were there corpora available for data-driven analysis and model
development.
Furthermore, the voice-based interaction nature requires the system to take
into account issues that are less severe in text-based chatbots, including
automatic speech recognition (ASR) errors, natural language understanding (NLU)
challenges such as sentence segmentation and disfluencies, natural language
generation (NLG) constraints with the use of the text-to-speech synthesis (TTS).
Moreover, as it is clear to users that they are speaking to a bot, the
conversation may involve much more commands, which are rarely observed in
existing human-human conversation corpora such as the Switchboard dataset
\cite{SwitchboardCorpus}.
Additionally, since users expect the bot to talk about recent events, the system
needs to dynamically update its knowledge about real world events.
Consequently, existing conversation corpora can hardly cover the full spectrum
of socialbot interactions.
With these challenges in mind, the Sounding Board system is initially built upon
intuitive hypotheses about socialbot conversations, which are then tested with
real users and improved based on user feedbacks over the course of the
competition.


==> chapter_3/_analysis.tex <==
To analyze system performance, we study conversation data collected from Sounding Board over a one month period
(Nov.~24--Dec.~24, 2017). 
In this period, Sounding Board had 160,210 conversations with users that lasted
3 or more rounds, where a round is defined as a user turn and the following
system turn.
We omit the shorter sessions, since many involve cases where the user did not
intend to invoke the system.
At the end of each conversation, the Alexa Prize platform collects a rating from
the user by asking {\it ``on a scale of 1 to 5, how do you feel about speaking
with this socialbot again?''} \cite{AlexaPrize2017}.
In this data, 43\% were rated by the user, with a mean score of 3.65
($\sigma=1.40$).
Of the rated conversations, 23\% received a score of 1 or 2, 37\% received a
score of 3 or 4,
and 40\% received a score of 5.
Some users give a fractional number score and these scores are rounded down to
the next smallest integer.
The data are used to analyze how different personality types interact with the
system in \cite{Fang2018NAACL}.\hfang{Revise}
and user engagement characteristics of the conversations
in \S\ref{chap3:ssec:insights_content}.

% \subsection{Content Analysis}
% \label{chap3:ssec:insights_content}

\begin{figure}
	\centering 
	%trim={<left> <lower> <right> <upper>}
	\includegraphics[width=0.8\textwidth,trim=1cm 0.5cm 1cm 1cm]{figs/percentBins20noTitle.png}
	\caption{Average conversation score by conversation length. 
		Each bar represents conversations that contain the number of rounds in the
		range listed beneath them and is marked with the standard deviation.
	}
	\label{fig:avg_score}
\end{figure}

We found that most Sounding Board conversations were short (43\% consist of
fewer than 10 rounds), but the length distribution has a long tail.
The longest conversation consisted of 772 rounds, and the average conversation
length was 19.4 rounds.
As seen in Fig. \ref{fig:avg_score}, longer conversations tended to get higher
ratings.

While conversation length is an important factor, it alone is not enough to
assess the conversation quality, as evidenced by the low correlation with user
ratings (Pearson $r=0.14$) and because some turns (e.g., repairs) may have a negative
impact.
Therefore, we carry out preliminary analysis for conversations of roughly equal
length (36--50) with high ratings (5) vs.~low ratings (1--2).
We automatically segment the conversations into subdialogs based on the
system-identified topic, similar to the three segments in
Table\,\ref{tab:sample_conversation}.
We then annotate each subdialog as engaged or not depending on whether there are
at least two user turns where the system detects a positive reaction.
A positive reaction can be accepting a proposal or a positive comment as
described in Table\,\ref{tab:user_reaction_frame}.
Then, we compute the percentage of engaged subdialogs in each conversation and
found that the average percentage differ significantly for high vs.~low scoring
conversations, i.e., 62.5\% for high vs.~28.6\% for low. 
This observation motivates us to develop a more robust metric than conversation
length that takes into account the fine-grained user engagement.


==> chapter_3/_dialog_context_tracking.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{l|p{13cm}}
		\hline\hline
		{\bf Attribute Set}  & {\bf Description} \\
		\hline
		% Reaction & User's reactions to the previous bot utterance. \\
		% Current topic & User's belief of the current discourse topic and its
		% associated information. \\
		% Personality & Personality questions that have been asked, and inferred trait
		% scores. \\
		% Topic history & Topics that have been discussed, suggested by the bot,
		% mentioned by the user.\\
		% Content history & Content that have been presented to the user. \\
		% Miniskill usage & Usage statistics of individual miniskills. \\
		Utterance 	& The meaning representation of the current user utterance. \\
		Personality & User's personality traits. \\
		Topic & The current topic and previously mentioned topics. \\
		Content & Content post history. \\
		Miniskill & Miniskill usage history. \\
		\hline\hline
	\end{tabular}
	\caption{Attributes in the multi-dimensional dialog context tracked by Sounding Board.}
	\label{tab:user_profile}
\end{table}

To serve the user-centric objective, Sounding Board maintains a
multi-dimensional user profile\hfang{change} such that it can adapt its responses and
strategies based on both immediate user reactions and accumulated knowledge of
the user.
Currently, Sounding Board tracks 5 sets of attributes as summarized in
Table\,\ref{tab:user_profile}.\hfang{change}
The utterance attribute set is updated by analyzing the current user utterance
from multiple aspects, including the intent, the question, the reaction, and the
topic.
More details about the utterance analysis will be provided in
\S\ref{chap3:sec:nlu}.
% The reaction attribute set is primarily updated by analyzing the user's
% utterance, e.g., detecting yes-no answers, agreement, and sentiment.
% More details about reaction analysis will be provided in
% \S\ref{chap3:ssec:user_reaction_analysis}.
The personality attribute set records the user's answer on personality questions
during the {\bf Ask Personality Questions} miniskill, which are converted to
scores on individual traits as described in \S\ref{chap3:ssec:personality}.
{\color{red}The remaining 3 sets are used to keep track of the user's mental states about
the conversation in terms of topics, content, and miniskills, respectively.
The topic attribute set records the history topic status, indicating whether a
topic has been discussed, suggested by the bot, or mentioned by the user.
It also records the current topic and its initiation context information, e.g.,
whether it is suggested by the bot or the user.
It further tracks the number of presented content posts about the current topic
after its initiation to estimate the user's interest level about the current
topic.
Similarly, the content attribute set and the miniskill attribute set tracks the
usage of content posts and miniskills in the conversation.
They are primarily used by the bot to avoid presenting duplicated content and
promote the diversity of conversation strategies.}\hfang{these are not mental
states}

In Sounding Board, the dialog context is reset at the beginning of the
conversation and constructed dynamically during the interaction.\hfang{no need}
We do not keep the user profile\hfang{change} across conversations since the device address is
not a reliable indicator of the user ID considering that each device may be used
by multiple users.
When speaker identification is available, maintaining long-term dialog context
for a user will be valuable for future work.\hfang{verify?}

{\color{gray}
Each miniskill manages a short conversation segment, which can be viewed as a
sequence of activity states.
% The dialog control for a miniskill is then formulated as a finite-state machine.
% Each state is implemented by a {\bf dialog agent}, following the naming
% convention in the Ravenclaw DM framework~\cite{Bohus2009CSL}.
To handle the complex dialog control for individual miniskills and smooth
transition between them in a socialbot conversation, we propose to use the
hierarchical dialog control.
\hfang{Maybe describe the knowledge graph here like Chapter~6?}

% Sounding Board carries out a long conversation by 
% assembling these miniskills
% with a coherent and engaging dialog plan\hfang{change} that is dynamically
% adjusted during the conversation.
% To adjust the dialog context plan\hfang{change}, we use a multi-dimensional
% dialog context tracking\hfang{change}.

% The multi-dimensional dialog context tracking is discussed in
% \S\ref{chap3:ssec:dialog_context}.
% Then, we discuss the hierarchical dialog control in
% \S\ref{chap3:ssec:dialog_control}.
% Finally, a sample conversation is analyzed in
% \S\ref{chap3:ssec:sample_conversation}.
}




==> chapter_3/_dialog_control.tex <==

Sounding Board uses a hierarchical dialog control\hfang{change} that involves
four levels: the conversation level, the topic level, the miniskill level, and
the turn level.
At the {\bf conversation level}, the discourse planning\hfang{change} primarily makes the
decision on the next topic when a topic switch action is triggered.
At the {\bf topic level}, the discourse planning\hfang{change} checks the miniskill usage for
the current topic and decides the next miniskill according to the usage history.

At the {\bf miniskill level}, the bot maintains a specific discourse
plan\hfang{change} for
each miniskill.
A typical miniskill discourse\hfang{change} has three stages, i.e., negotiation, execution,
and termination.
In the negotiation stage, the bot confirms with the user to start the miniskill
on a chosen topic.
Note the bot does not always need to negotiate with the user before executing
the miniskill.
The execution stage can involve multiple turns and the bot {\color{red}dynamically adjusts
the discourse plan}\hfang{change} according to the user's responses and available content.
At the termination stage, the bot checks whether the user wants to continue the
miniskill/topic via explicit confirmation.
If the user wants to continue, the bot can return to the execution stage.
Sometimes the bot does not confirm with the user and directly terminates the
miniskill with an explanation.
For example, if the user is clearly bored or there is no content or action left
for the discourse plan.\hfang{change}
\hfang{give explanation, examples for these cases}

Finally, at the {\bf turn level}, the bot assembles a response by organizing a
sequence of dialog acts.\hfang{response plan?}
The dialog acts are realized via templated utterances.
To increase the diversity, we create multiple templates for each dialog act.
We also make extensive use of speech synthesis markup language (SSML) for
prosody and pronunciation to convey information more clearly.
They are used to improve the naturalness of concatenated dialog acts, to
emphasize suggested topics, to deliver jokes more effectively, to apologize or
backchannel in a more natural-sounding way, and to more appropriately pronounce
unusual words.\hfang{that are part of the back story or personality quiz}

The hierarchical dialog control\hfang{verify} simplifies updating and adding
new capabilities. 
It is also useful for handling high-level conversation mode changes that are
frequent in user interactions with socialbots.
In general, Sounding Board has three key objectives for the discourse
planning\hfang{change} at all levels: coherence, diversity.\done{remove
proactivity}.
The bot tries to maintain {\bf coherence} by choosing content on the same or a
related topic within a conversation segment.
It also avoids presenting topics or content that were already shared with the
user.\hfang{avoid repetitive is diversity, not coherence}
The {\bf diversity} objective aims to maintain user interest by promoting
different miniskills where the interaction strategies and content types differ.
{\color{red}Finally, the {\bf proactivity} objective makes the bot actively suggest
relevant activities or topics during the conversation.
For example, when the user asks a question, the bot does not only give the
answer but also suggests some relevant content about a topic extracted from the
question.
Similarly, when the user initiates a topic which the bot does not have any
content about, the bot would try to suggest a relevant topic to continue the
conversation.}\hfang{change to mixed-initiative: suggestive?}



==> chapter_3/_discussion.tex <==
\begin{itemize}
	\item Sounding Board from the perspective the user modeling. The user's
		expertise or interests affect the discourse planning.
		Additionally, user reactions. See NLU pre-processing.
		Also, personality questionnaire.
	\item Challenges about the evaluation?
\end{itemize}


==> chapter_3/_inbox.tex <==
First, the bot is {\bf user-centric}.
It negotiates with the user about the activity and topic.
It also attempts to probe the user's personality and establish trust with the
user through a subdialog of getting to know each other.
During the conversation, the bot actively acknowledges users to reflect its
understanding of their mental states, e.g., sentiment, frustration, and opinion.
The information about their mental states and personalities are used to adjust
the bot's topic choice and interaction strategy.
The bot is also {\bf content-driven}.
It supplies interesting and relevant information to continue the conversation,
enabled by a rich and daily updated content collection.
With this content, the bot can actively drive the conversation forward and
engage users for a long period of time.

We organize them into two types based on their discourse complexity.
{\bf Basic acts} are always fulfilled within a single bot turn, whereas {\bf
composite acts} span multiple continuous user and bot turns.
{\color{red}The conversation act is instantiated by the bot according to the
context of the conversation.
Expand on the Bot Knowledge?}

{\bf Basic acts} refer to passive bot actions that acknowledge user
utterances or resolve (either successfully or unsuccessfully) one-shot user
requests.
These acts are always fulfilled within a single bot turn.
In contrast, {\bf shallow acts} can involve multiple user and bot turns.
They can be initiated either explicitly by the user or proactively by the bot.
Within a shallow act, the bot usually performs a mixture of customized request
and inform acts, as well as those basic acts.
{\color{red}Among the shallow acts described in Table\,\ref{tab:conversation_acts}, the act
of sharing knowledge \dots.
The knowledge is unstructured/shallow knowledge.}
Finally, structured \dots.
{\bf hierarchical acts} maintain complex discourse structures where the
bot may perform proper shallow acts in addition to basic acts and customized
request and inform acts.
For example, during a movie discussion, the bot may suggest relevant subtopics
(e.g., the director of the movie) and start sharing knowledge about a subtopic.

{\bf Basic acts} are always fulfilled within a single bot turn, and a bot turn
may consist of multiple basic acts.
In contrast, {\bf shallow acts} involve multiple continuous user and bot turns.
They maintain relatively simple discourse structures, i.e., there is no embedded
shallow acts under a shallow act.
Finally, {\bf hierarchical acts} maintain complex discourse structures which
can span multiple shallow acts in addition to basic acts.
In particular, Sounding Board implements two hierarchical acts.
For example, during a movie discussion, the bot may suggest relevant subtopics
(e.g., the director of the movie) and start sharing knowledge about a subtopic.

While \dots acts are relatively easier to implement/statically encoded/available
APIs,
knowledge/content are dynamically and large scale.
Content sources: 
- Reddit (\texttt{TodayILearned}, \texttt{ShowerThoughts}, \texttt{LifeProTips})
- Jokes (Cached from Evi.com)
- News (\texttt{News}, \texttt{WorldNews}, \texttt{Politics},
\texttt{Technology}, \texttt{Science}, \texttt{Futurology},
\texttt{Sports}
- Movies (IMDb, Wikipedia) 

\begin{table}[t]
	\centering
	\begin{tabular}{c|c|p{6cm}}
		\hline\hline
		{\bf Act Type} & {\bf Conversation Act}  & {\bf Description} \\
		\hline
		Basic
		& Acknowledge User Utterances & \\
		& Ask For Confirmation & \\
		& Ask Personal Questions & \\
		& Ask Factual Questions & \\
		& Inform Bot Knowledge & Answer personal/factual questions \\
		& Repeat Last Bot Utterance & \\
		& Provide Help Messages 		& \\
		\hline
		Composite
		& Warm Up & Welcome and greet the user 	\\
		\cline{2-3}
		& Probe User Personality 		& get-to-know-each-other, via personal perference
		questions, and share its own answer \\
		\cline{2-3}
		& Suggest/Negotiate Chat Topic(s) & \\
		& Discuss A Topic & \\
		% & Exchange Knowledge about a Topic		& TIL, SHS, LPT, Jokes,
		% Definition, SQuAD, Movie Metadata?, News \\
		% % & Ask Factual Questions about a Topic & SQuAD with question/answer \\
		% \hline
		% Hierarchical
		% & Discuss Movies 				& \\
		% & Discuss News Articles & \\
		\hline\hline
	\end{tabular}
	\caption{Sounding Board's coarse-grained conversation acts.}
	\label{tab:conversation_acts}
\end{table}
\begin{table}[t]
	\centering
	\begin{tabular}{c|c|p{6cm}}
		\hline\hline
		{\bf Life Span} & {\bf Conversation Act}  & {\bf Description} \\
		\hline
		Turn-level
		& Confirmation 					& \\
		& Knowledge of Content 					& \\
		& Attitude to the content/bot   & \\
		& Opinion stance about \dots & \\
		\hline
		Conversation-level
		& Personality Type & \\
		& Discussed Topics & \\
		\hline\hline
	\end{tabular}
	\caption{The user profile maintained by Sounding Board during the conversation.}
	\label{tab:user_profile}
\end{table}

The system engineering strategy is driven by the lack of appropriate
conversational data for training and the plan to use multiple content sources,
which together motivate a modular architecture with a hierarchical dialogue
management strategy. As new capabilities are developed, it is relatively
straightforward to add them to the system, and the modular architecture also
easily scales to handle more miniskills and facilitates updating components as
more useful data becomes available for data-driven learning.
The generation strategy is also modular, with different components for different broad categories of speech acts.
In order to make the conversational data currently being collected more useful
for dialogue policy learning (and to make the system less monotonous), the
response generation module includes several mechanisms for randomly introducing
variation, and the randomness associated with content availability for different
topics also leads to potentially useful variation in the conversations.

In order to make the conversational data currently being collected more useful
for dialogue policy learning (and to make the system less monotonous), the
response generation module includes several mechanisms for randomly introducing
variation, and the randomness associated with content availability for different
topics also leads to potentially useful variation in the conversations.
The Sounding Board design philosophy is primarily reflected in the conversation
strategy and the system engineering approach.
The conversation strategy has two key features. 

Sounding Board uses a modular framework as shown in Fig.\,\ref{fig:system_arch}.
When a user speaks, the system produces a response using three high-level modules: 
natural language understanding (NLU), dialog manager (DM), and natural language
generation (NLG).
{\color{red}(To be updated.)}

Sounding Board interacts with users through Amazon's Automatic Speech
Recognition (ASR) and Text-to-Speech (TTS) APIs included in 
the Alexa Skill Kit (ASK)\footnote{\url{https://developer.amazon.com/alexa-skills-kit}}
which acts as the front-end of Sounding Board.
The NLU produces a representation of the current event by analyzing the user's speech given the current dialog state (\S\ref{ssec:nlu}).
Then, based on this representation, the DM executes the dialog policy and
decides the next dialog state (\S\ref{ssec:dm}). 
Finally, the NLG uses the content selected by the DM to build the response (\S\ref{ssec:nlg}),
which is returned to the user and stored as context in the DM.
During the conversation, the DM also communicates with a knowledge graph 
that is stored in the back-end and updated daily by the content management module (\S\ref{ssec:content}).
The system is deployed as an AWS Lambda service triggered by ASK events, which
contain the ASR hypotheses for a user utterance and the output of the voice user
interface (VUI) which identifies selected user intents.
The AWS Lambda service acts as the middle-end of Sounding Board.
As shown in Fig.\,\ref{fig:system_arch}, it consists of three major system
modules of Sounding Board:
a natural language understanding (NLU) module,
a dialog management (DM) module,
and a natural language generation (NLG) module.
These system modules also communicate with different back-end services,
including:  
a Stanford CoreNLP server \cite{CoreNLP} deployed at AWS EC2 for providing the
parsing service,
AWS DynamoDB tables where the content (knowledge graph) are stored,
and Evi.com\footnote{\url{https://www.evi.com}} for providing a question
answering service.

Upon receiving an ASK event, Sounding Board goes through the three major system
modules to produce a response to be returned to the ASK.
First, the NLU module produces an input frame for the current event by analyzing
the ASR hypotheses, the VUI output, and the dialog state.
Then, the DM module examines the input frame, executes the dialog policy, and updates the dialog state. 
The DM operates at two levels, with a master to manage the overall conversation and a collection of miniskills 
to handle different types of conversation segments (discourse segments).
Finally, the NLG module uses the speech act and content selected by the DM module to build the response,
which is returned to the ASK and also stored as part of the conversation context in the DM module.


\subsection{Dialog Management}\label{ssec:dm}
%As shown in Fig.\,\ref{fig:system_arch}, 
%The DM extensively communicates with other modules.
% Sounding Board has three high-level dialog policies: 
We designed the DM according to three high-level objectives: 
 engagement, coherence, and user experience.
%The {\bf engagement} principle ensures 
The DM takes into account user {\bf engagement} based on components of the NLU output 
% estimates user engagement based on the NLU output and 
and tries to maintain user interest by promoting diversity of interaction strategies (conversation modes).
Each conversation mode is managed by a miniskill
%\noah{too many italics/boldfacing in this paragraph, do these things all need to be treated as special terms?}
that handles a specific type of conversation segment.
The DM tries to maintain dialog {\bf coherence} by choosing content on the same or a related topic within a conversation
segment,
and it does not present topics or content that were already shared with the user.
To enhance the {\bf user experience}, the DM uses conversation grounding acts to
explain (either explicitly or implicitly) the system's action and to instruct the
user with available options.

%\footnotetext{included in the Alexa Skill Kit (ASK) \url{https://developer.amazon.com/alexa-skills-kit}}

The DM uses a hierarchically-structured, state-based dialog model
operating at two levels:
a master that manages the overall conversation, 
and a collection of miniskills
%(summarized in Appendix\,\ref{ssec:miniskill_details}) 
that handle different types of conversation segments. 
This hierarchy enables variety within specific topic segments.
%a conversation on a single topic.
In the Fig.\,\ref{fig:sample_convo} dialog,
%in Fig.\,\ref{fig:sample_convo},
Turn\,3 was produced using the \textit{Thoughts} miniskill, 
Turn\,4 using the \textit{Facts} miniskill,
and Turns\,5--7 using the \textit{Movies} miniskill. 
% (discourse segments)
%A master processing sequence manages the conversation as a whole, and a collection of {\it miniskills} (summarized in Table\,\ref{tab:miniskills}) that manage conversation segments for specific conversation modes.
The hierarchical architecture simplifies updating and adding new
capabilities. 
It is also useful for handling high-level conversation mode changes
that are frequent in user interactions with socialbots.

At each conversation turn, a sequence of processing steps are executed to identify a response
strategy that addresses the user's intent and meets the constraints on the
conversation topic, if any.
First, a state-independent processing step checks if the speaker is initiating a new conversation segment (e.g., requesting a new topic). 
If not, a second processing stage executes state-dependent dialog policies.
Both of these processing stages poll miniskills to identify which ones are able
to satisfy constraints of user intent and/or topic. 
Ultimately, the DM produces a list of speech acts and corresponding content 
to be used for NLG, and then updates the dialog state.


\subsection{Natural Language Generation}\label{ssec:nlg}

The NLG module takes as input the speech acts and content
provided by the DM and constructs a response by generating and
combining the response components.


\noindent
% {\bf Speech Act Realization}:\hfang{TBD: Update the system arch figure.}
{\bf Phrase Generation}:
The response consists of speech acts from four broad categories:
grounding, inform, request, and instruction.
For instance, the system response at Turn\,7 contains three speech acts: grounding
({\it ``Interesting.''}), inform (the IMDb rating), 
and request ({\it ``do you like the movie's director?''}). 
% Details about individual speech acts are provided in the supplementary
% materials.
As required by the hosting platform,
the response is split into a message and a reprompt.
The device always reads the message;
the reprompt is optionally used if the device does not detect a response from the user.
The instruction speech acts are usually placed in the reprompt.

\noindent
{\bf Prosody}:
We make extensive use of speech synthesis markup language (SSML) for
prosody and pronunciation to convey information more clearly.
%better convey the information our bot wishes
%\noah{I don't like this attribution of wishes to the bot ...}
%\hfang{how about ``intends''?}
%\ari{+1 for intends}
%\eclark{I'd change it to: ``to convey information more clearly.''}
%
to communicate.
We use it to improve the naturalness of concatenated speech acts, to emphasize suggested topics, to deliver jokes more effectively,
to apologize or backchannel in a more natural-sounding way,
and to more appropriately pronounce unusual words.

\noindent
{\bf Utterance Purification}:
% \eclark{If we're short on space, this can go.}
The constructed response (which may repeat a user statement) goes through an utterance purifier
%\footnote{We use the nodejs-profanity-util package (\url{https://github.com/KanoComputing/nodejs-profanity-util}) with a profanity word list merged from multiple sources.}
that replaces profanity with a non-offensive word chosen randomly from a list of innocuous nouns, often to a humorous effect.
% The purifier is needed since the constructed response may contain part of the
% recognized user utterance and content retrieved from online sources, either of
% which may include profanity.
%Some of the word replacements have an amusing result.

\subsection{Content Management}\label{ssec:content}

% Content acquisition and management are two important steps towards implementing
% a successful content-oriented miniskill.
Content is stored in a knowledge graph at the back-end, which is updated daily.
The knowledge graph is organized based on miniskills so that 
query
% entity grounding
%\mari{I don't know what entity grounding means here.}
%\chenghao{changed to ``query''. It means we can retrieve contents efficiently when user initiates a topic.}
and recommendation can be carried out efficiently by the DM.
The DM drives the conversation forward and generates 
%%MO: I don't think this is a correct use of "grounded"
%grounded 
responses by
either traversing links between content nodes associated with the same topic or through relation edges
to content nodes on a relevant new topic.
%\mari{Reworded to indicate that there are two types of links. Hao C should check and revise if needed.}
The relation edges are compiled based on existing knowledge bases (e.g., Wikipedia and IMDb) and entity co-occurrence between content nodes.

% Sounding Board acquires content from multiple sources, including online
% user-generated contents and news articles on Reddit\footnote{Reddit posts come with user votes,
% which we can use to identify content that is of higher interests. News articles
% are daily updated.},
% movies from IMBD, question-answer pairs from the SQUAD dataset \cite{SQUAD2016},
% and jokes crawled from Evi.com.
% The specific sources are chosen because we felt that there was news or
% commentary that many people would appreciate in a style that was reasonably well
% suited to spoken conversations. 
% In addition,  we needed it to be easy to extract short snippets of information
% that is informative and requires little context to understand.

% \noindent
% {\bf Knowledge Graph Construction}:
% The knowledge graph of our system is to organize the web text content such that
% two tasks , entity-grounding and recommendation, can be carried out efficiently.
% Firstly, We compile explicit relation knowledge from existing knowledge base
% that aligns well with our content source, such as Wikipedia, IMDb and GoodReads.
% Secondly, the complied knowledge graph is extended with implicit relation
% knowledge relying on the entity co-occurrence within certain span range in our
% content source. During the conversation, a topic entity leads our system to land
% on the corresponding graph node and the dialog manager then can utilize the
% neighboring knowledge graph to drive the conversation forward and generate
% grounded response, by either traversing the relation edge to another topic or
% retrieving the relevant text content.

Because Sounding Board is accessible to a wide range of users, the system needs to provide content and topics that are appropriate for a general audience.
% \eclark{Again, if we're short on space, cut this paragraph down or delete.}
This requires filtering out inappropriate and controversial material.
%from the knowledge graph.
Much of this content is removed using regular expressions to catch profanity. 
However, we also  filtered content containing phrases related to sensitive topics
or phrases that were not inherently inappropriate but were often found in
potentially offensive statements (e.g., ``your mother''). 
% The goal of the content filtering was recall rather than precision; we leave
% exploring more precise methods of content filtering to future work.
% Therefore, three types of contents are filtered:
% 1) content with profanity,
% 2) content covering controversial or offensive topics,
% and 3) content triggering uncomfortable or depressing feelings.
%TTS-unfriendly content (e.g., URLs and lengthy content) is either removed or simplified.
Content that is not well suited in style to casual conversation (e.g., URLs and lengthy content) is either removed or simplified.


While more specific relations beyong \texttt{Mentions} and \texttt{MentionedIn}
are desirable, we leave it as future work.
First, enriching the relations requires stronger language understanding and
information extraction capabilities across multiple domains.
Second, the socialbot needs to customize the way to naturally inform the
relation for individual relation types. 






\begin{table}[t]
    \centering
    \caption{Personality type to Disney character mappings.}
    \label{tab:disney}
    \begin{tabular}{ccl}
    \toprule
        \textbf{Openness} & \textbf{Extraversion} & \textbf{Character}\\ \midrule
        $-$ & $-$ & Aladdin, Snow White \\
        $-$ & $+$ & Kristoff (\textit{Frozen}), Marlin (\textit{Nemo})\\
        $+$ & $-$ & Elsa (\textit{Frozen}), Belle (\textit{Beauty and the Beast}) \\
        $+$ & $+$ & Ariel (\textit{The Little Mermaid}), Anna (\textit{Frozen})\\
        \bottomrule
    \end{tabular}
\end{table}




==> chapter_3/_trash.tex <==
With these challenges in mind, the Sounding Board system is initially built upon
intuitive hypotheses about socialbot conversations, which are then tested with
real users and improved based on user feedback over the course of the
competition.

We argue that it is extremely crucial for socialbots to have access to
up-to-date content that are useful for social chat.
Therefore, the two popular approaches used for chit-chat systems,
i.e., scripting responses with template-matching rules (e.g.,
ELIZA~\cite{Weizenbaum1966Comm}, ALICE~\cite{Wallace2009ALICE})
and retrieving responses from a large scale conversation repository (e.g.,
\cite{Jafarpour2009NIPS,Wang2013EMNLP,Sordoni2015NAACL,Yan2016ACL}), are not
adequate for socialbots.
In the former approach, it is \dots at scale,  and dynamically.
For the latter approach, injecting the knowledge is an open question.
\hfang{Rewrite this section}

		% 15 & User & {\it yes but let's chat about something else i want to talk
		% about science} \\
		% 16 & Bot 	& {\it Science ? I love it! Have you read this article from Last
		% Friday? The title was: U.S. Report Says Humans Cause Climate Change,
		% Contradciting Top Trump Officials.} \\
		% 17 & User & {\it oh yeah} \\
		% 18 & Bot 	& {\it Cool! This news talked about climate. Would you like to
		% 	hear some advice my friend gave to me about that?} \\
		% 19 & User & {\it how many stars in the universe?} \\
		% 20 & Bot 	& {\it The universe has 70,000,000,000,000,000,000,000 stars. Do
		% you still wanna to hear some advice my friend gave to me about climate?} \\
		% 21 & User & {\it no thank you}\\
		% 16 & Bot 	& {\it Science ? I love it! Have you read this article from Last
		% 	Friday? The title was: Texas Engineers Develop New
		% Material for Better Lithium-Ion Batteries.} \\
		% 17 & User & {\it oh yeah} \\
		% 18 & Bot 	& {\it  Cool! This news talked about batteries. Do you wanna hear
		% this random thought I had about that?}\\
		% 19 & User & {\it sure} \\
		% 20 & Bot 	& {\it  Great! You know what I realized the other day? Putting an
		% ice pack in the freezer is like charging it's frosty batteries.} \\
		% 21 & User & {\it you are weird alexa} \\
		% 22 & Bot 	& {\it Yeah. It probably doesn't make sense. Have you read this
		% 	article from Last Wednesday? The title was: What to worry about when
		% 	you're worrying about lithium-ion batteries -- We're living in a time when
		% new technology is extremely material-dependent.} \\
		% 23 & User & {\it no i did not} \\
		% 24 & Bot 	& {\it Ummm. Let's see. That news mentioned technology. Do you
		% wanna know an interesting fact about that?} \\
		% 25 & User & {\it no thanks stop} \\

alexa let's talk about universal studios (0.421) ||| hey alexa let's talk about
universal studios (0.098) ||| alexa good let's talk about universal studios
(0.033) ||| hey alexa good let's talk about universal studios (0.008) ||| a
alexa let's talk about universal studios (0.053)	 I think you'd like to hear
what I have to say about universal studios. You know what I realized the other
day? Universal Studios logo only shows Earth, though it should probably show the
whole universe. . <break time="100ms"/> 
oh you're so right (0.592) ||| oh oh you're so right (0.140) ||| oh oh you're so
right (0.108) ||| oh you're are so right (0.085) ||| oh we so right (0.092)
Umm, <break time="50ms"/>  My friend in the cloud asked me this question. What
notable female star left Universal after the Standard Capital takeover? <break
time="100ms"/> 
i don't know (0.777)	 The answer is, <break time="50ms"/>  <prosody
rate="slow">Margaret Sullavan .</prosody>  <break time="50ms"/>  I learned from
the web that in 1994 when the Power Rangers went to Universal Studios, it caused
an 8 mi. long traffic jam in L.A. . <break time="100ms"/> 
wow that's incredible (0.614)	 Hmm. <break time="50ms"/>  Would you like to continue our  conversation on universal studios?
no (0.879)	 We've chatted for a bit, <break time="50ms"/>  I'd like to get to
know you, is that okay?

% {\bf User Profile Update Stage}:\hfang{change}
% First, the master DM updates the user profile based on the incoming user
% utterance.
% While some attributes can be updated by the master DM itself, the update logic
% of several attributes is miniskill-dependent.
% Thus, these attributes are updated by the internal logic of the active miniskill.
% Meanwhile, if a chat command is detected in the user's utterance, the master DM
% can terminate the previous active miniskill. 

% {\bf Active Miniskill Execution Stage}:
% In this stage, the master dialog manager let the miniskill dialog manager of the
% active miniskill to take the dialog control.
% Depending on the progress of the miniskill, it may become completed if it has
% finished its dialog flow.

% {\bf Miniskill Polling Stage}:
% The bot should always have an active miniskill that is in charge of the current
% turn.
% Therefore, if the previous active miniskill is terminated for some reason, the
% master dialog manager needs to poll miniskills with one or multiple candidate
% topics.
% Depending on the dialog context and the polling results,
% the master dialog manager can decide whether to start a new topic or continue on
% the previous one.
% Afterwards, the master dialog manager makes one miniskill active to continue the
% conversation.
% The miniskill polling and selection processes take into account the dialog
% context and/or the attributes specified in the user's commands.
% Content selection
% \hfang{how? where does content selection come in? is that part of the miniskill
% ranking or separate?}


==> chapter_4/_conclusion.r2.tex <==
This work has provided in-depth analyses of agent, content, and user factors 
for evaluating long socialbot conversations.
We characterize user factors via intents, fine-grained engagement,
speaking style, language use, and user personality.
Experiments show that user factors, especially user engagement, are 
among the most informative about user ratings.
In addition, our results indicate that user personality is useful 
for both predicting user ratings and understanding user topic preferences.
However, much of the data do not have personality information,
suggesting a future direction of learning a proxy by clustering user
conversation histories. 

\begin{comment}
We approach the rating sparsity problem by estimating ratings 
at multiple levels: conversation, subdialog, and microsegment.
Estimated subdialog ratings are validated through human evaluation.
Microsegment ratings aggregated across conversations can also 
provide diagnostics about dialog policy. %at system level.
In an analysis of a topic initiation policy points to the advantage of
maintaining relevance in topic transitions.
A future direction is to use the learned reward functions in
reinforcement learning to improve the dialog policy.
\end{comment}

We further demonstrate two approaches to estimate rewards at multiple levels.
The learned linear and BiLSTM reward functions significantly outperform the
baseline models for conversation-level rating prediction.
Additionally, the subdialog rewards have much higher correlations with human
judges compared with length-based and conversation-rating-based reward
functions.
Additionally, we provide examples showing how segment-level rewards can be used
to diagnose system performance in terms of topic identification, topic
initiation policy, and content sources.



==> chapter_4/_correlation_analysis.tex <==
\begin{comment}
Two hand-crafted metrics are created based on the observation using user dialog
acts and bot conversation acts, respectively.\hfang{why not \%?, probably should add
them, but they ignore \# turns, which I think is important}

\begin{tabular}{ll}
	$f$\textsubscript{user} = 
	& \#\texttt{FollowAndNonNegative} 
	$+$ \#\texttt{AcceptTopic} \\
	& $+$ \#\texttt{InterestedInContent}
	$+$ \#\texttt{PositiveToContent} \\
	& $-$ \#\texttt{RejectTopic}
	$-$ \#\texttt{NotInterestedInContent} \\
	& $-$ \#\texttt{NegativeToContent} \\

	$f$\textsubscript{bot} = 
	& \#\texttt{ConfirmToContinue} 
	$+$ \#\texttt{DiscussTopic}
	$-$ \#\texttt{NegotiateTopic}
\end{tabular}

\noindent
The correlation coefficients for $f$\textsubscript{user} and
$f$\textsubscript{bot} are ? and 0.20, respectively.
\end{comment}


==> chapter_4/_exp.features.tex <==
\noindent
{\bf Correlation analysis}:
Fig.\,\ref{fig:feature_correlation} shows the correlations between a subset of
factors (represented as percentage of turns or topics) 
and conversation-level user ratings.
The correlations are computed on the training set.
As expected, positive user reactions and intents have positive correlations, and
vice versa.
For example, U12 (user engaged turns) is the most positively correlated
factor, whereas U9 (user expresses no interest in further discussion) is
the most negatively correlated factor.
For agent factors, the agent's inability to accommodate a user request is a
negative sign.
Specifically, A1 (negotiation) and A4 (apology)
% \maarteninline{I rephrased this:}
reflect costly conversation turns
%%MO: this sounds like a constraint on the set of turns, and I don't think that's what you mean so I rewrote
%after the user expressed 
(i.e., associated with dissatisfaction), 
% negatively impacts user ratings since they increase the cost of socialbot conversations,
whereas A2 (topic discussion) has positive correlation since those are efficient turns in the conversation.
For content-related factors, topics initiated by rejecting the user topic (T3)
or extracted from a non-topic-initiation user utterance (T4) are negatively
correlated with user ratings.

\begin{figure}[t]
	\centering
	%trim={<left> <lower> <right> <upper>}
	\includegraphics[width=0.9\textwidth]{figs/feature_corr.pdf}
	\caption{Correlation (Pearson $r$) between a subset of factors and conversation-level user ratings. All results are statistically significant (p $\ll$ 1e-5).} 
	\label{fig:feature_correlation} 
\end{figure}


\begin{table}[t]
	\centering
	\begin{tabular}{l|c|c|c|c}
		\hline\hline
		{\bf Feature Groups} 
		& $|\mathcal{F}|$
		& {\bf $r$} 
		& {\bf $\rho$} 
		& {\bf $R^2$} \\
		\hline
		%%%%% baselines %%%%%
		% Random & 0 
		% & 0.8 & 0.8 & -122.3 \\
		% & .01 & .01 & -1.22 \\
		%%%%
		% NumTurns & 1 
		% & 12.9 & 15.1 & 1.6 \\
		% & .13 & .15 & .02 \\
		% \hline
		%%%%% agent %%%%%
		%%%%
		F1-AgentAct & 61
		% & 24.3 & 22.5 & 5.9 \\
		& .24 & .23 & .06 \\
		%%%%
		F2-AgentBoW & 6k+
		% 6137
		% & 25.9 & 23.4 & 6.7 \\
		& .26 & .23 & .07 \\
		\hline
		%%%%% topic %%%%%
		F3-Coherence & 6
		% & 11.9 & 13.6 & 1.4 \\
		& .12 & .14 & .01 \\
		F4-TopicContext & 15
		% & 13.2 & 11.4 & 1.7 \\
		& .13 & .11 & .02 \\
		%%%%
		F5-BagOfTopics & 7k+
		%7080
		% & 14.1 & 12.5 & 2.0 \\
		& .14 & .13 & .02 \\
		%%%%
		\hline
		%%%%% user %%%%%
		F6-UserVerbosity & 2
		% & 16.8 & 17.3 & 2.8 \\
		& .17 & .17 & .03 \\
		%%%%
		F7-UserReaction & 33
		% & 25.8 & 23.7 & 6.6 \\
		& .26 & .24 & .07 \\
		%%%%
		F8-UserBoW & 4k+
		%4658
		% & 29.9 & 28.3 & 8.9 \\
		& .30 & .28 & .09 \\
		\hline
		%%%%
		F1 -- F2 Agent & 6k+
		% & 27.4 & 25.6 & 7.5 \\
		& .27 & .26 & .08 \\
		%%%%
		F3 -- F5 Content & 7k+
		% & 22.0 & 19.8 & 4.8 \\
		& .22 & .20 & .05 \\
		%%%%
		F6 -- F8 User & 4k+
		% & {\bf 31.8} & {\bf 30.1} & {\bf 10.0} \\
		& {\bf .32} & {\bf .30} & {\bf .10} \\
		%%%%
		F1 -- F8 All & 17k+
		% & 31.7 & 29.5 & 10.0 \\
		& .32 & .30 & .10 \\
		\hline\hline
	\end{tabular}
	\caption{Validation set results for conversation-level rating regression using
		different predictor groups.
	}
	\label{tab:exp_conversation_level_validation}
\end{table}

\noindent
{\bf Regression analysis}:
Finally, we compare different factors by examining their conversation-level
rating regression performance using LASSO regression models.
The validation set results are shown in Table\,\ref{tab:exp_conversation_level_validation}.
% We use a linear regression model trained with $\ell_1$-regularization, i.e.,
% LASSO.
% The regularization penalty is tuned based on the root-mean-squared-error of the
% validation set.
We report the size of the feature set $|\mathcal{F}|$, as well as 
Pearson $r$, Spearman $\rho$, and $R^2$ on the validation set.
Note low $R^2$ is expected due to the high variance of user ratings.
% As expected, the number of turns alone is not very successful, although
% it outperforms the random baseline.
User-related factors (F6--F8) significantly outperform both agent-related
factors (F1--F2) and content-related factors (F3--F5).
Lastly, as shown by the last row, merging all three factor groups does not give
additional gain over user factors alone. %, indicating that user factors capture most information about user ratings.
This indicates that user reactions, intents, and language use contain the most
useful information for predicting the final conversation-level user ratings.


==> chapter_4/_intro.r3.tex <==
Engaging users in long, open-domain conversations with a chatbot remains a
challenging research problem.
Unlike task-oriented dialog systems which aim to accomplish tasks quickly, users
expect a broader variety of experiences from conversational chatbots (e.g.,
companionship, discussing recent news, or entertainment).
Differences in the nature of the two types of dialogs lead to different approaches to assessing system performance, a critical part of system development. 
When the system is designed to serve explicit goals, task completion time and success rate can be used, but user satisfaction is often the primary objective of a chatbot.

\begin{figure}[!t]
	\centering
	%trim={<left> <lower> <right> <upper>}
	\includegraphics[width=0.46\textwidth]{figs/intro_example.pdf}
	\caption{
		{\bf Left}: A conversation-level rating (2.5/5) does not paint a full picture of
		how individual dialog segments went.
		The first two agent turns were very well received by the user,
		whereas the last turn was less well received.
		% this information is not reflected by the 2.5/5 rating.
		{\bf Right}: The conversation can involve multiple topics and a discussion 
		on one topic can spawn a discussion of other related topics.
		To maintain such structure, the agent uses a stack-based topic tracking module 
		that provides a topic segmentation of the dialog. 
		% The underlying stack-based topic tracking for multi-level
		% segmentation.
		% The user initiates a topic ``science,'' and the agent initiates two spawned
		% topics ``milky way'' and ``trees.''
		Posts p1 and p2 are shown as underscored sentences. 
	}
\label{fig:intro_example}
\end{figure}



%\hfang{Should we explicitly mention the Alexa Prize socialbot's goal?
%`... to build and test \textit{socialbots}, i.e., a type of open-domain dialog systems (primarily) for chatting about popular topics and recent news''.}
The recent Alexa Prize \cite{AlexaPrize2017} has provided a new platform 
for researchers to build and test such open-domain chat-oriented dialog systems, i.e.,
\textit{socialbots}, by allowing systems to interact with millions of real users
through Alexa-enabled devices.
The platform provides an opportunity for getting real user feedback
at a very large scale, but some challenges remain.
First, users only give a single rating at the end of the conversation, and many
conversations are unrated.
For long conversations, an optional end-of-conversation rating is a weak signal
for learning dialog policies.
As shown on the left side of Fig.\,\ref{fig:intro_example}, a conversation can contain both good and bad segments.
Thus, conversation-level ratings do not uniformly apply to individual
segments.
%This challenge is shared by all dialog systems, but it is especially critical for
%socialbots involving long conversations.
Since it is impractical to ask a large number of users to rate their experience at the subdialog level,
it is crucial to understand conversation characteristics that reflect the user experience. 
In this paper, we carry out analyses of factors related to three aspects of socialbot conversations (agent, user, and content) in terms of how well they predict conversation-level ratings. We then introduce and assess two multi-level models for leveraging these features to predict ratings of different types of dialog segments.

Our contributions are three-fold.
First, using 68k rated conversations collected from a stable version of an Alexa
Prize socialbot, we carry out in-depth analysis of three aspects of
socialbot conversations: factors relating to the agent utterances and their
dialog acts, factors that capture topic coherence, and user factors that include
both fine-grained engagement indicators and user personality estimated by our
system using the five-factor model \cite{costa1992revised}.
The study
finds that user-related factors 
are most informative for predicting conversation-level ratings, and it sheds light on how users' personality types affect
their ratings and the kinds of topics they initiate.
Second, we explore two methods for estimating rewards at multiple levels, using local segment features with and
without a sequence model to capture dialog context. 
We show that predicted conversation-level rewards from both models are competitive with prior methods and that 
the derived segment rewards have higher correlation with human judges than uniform assignment of oracle conversation-level user ratings. Lastly, we provide three examples showing how the segment-level rewards can be used
to diagnose system performance.


==> chapter_4/_related_work.r2.tex <==
For task-oriented dialog systems, PARADISE \cite{Walker1997ACL} is a widely
adopted model-based evaluation framework, which focuses on  task cost and
success metrics.
It has been used for conversation-level user rating prediction
\cite{Walker2000NLE}, as well as optimizing dialog policy under a reinforcement
learning setting \cite{Rieser2011CL}.
For open-domain chatbots, reference-based evaluation is common
\cite{Sordoni2015NAACL,Shang2015ACL,Vinyals2015ICML,Serban2016AAAI,Li2016NAACL,Li2016ACL,luan2017multi,Ghazvininejad2018AAAI}.
Reference-based metrics (such as BLEU) are simple to compute, but they cannot account for fact that responses with completely different meanings can be equally acceptable, and they are unrelated to user satisfaction.
A model-based evaluation for system responses is
proposed by \citet{Lowe2017ACL} as an alternative to reference-based metrics.
\citet{Venkastech2017NIPS} use a variety of features with deep neural networks
and ensemble models to predict conversation-level user ratings.
\citet{Guo2017NIPS} study topic-based evaluation for socialbots 
by training a topic classifier.
Our work differs from these in that 
1) we study multiple aspects of socialbot conversations, i.e., agent, user, an content, and
2) we use a system-maintained topic stack to obtain topic segments for computing segment-level rewards.

% Dialog systems are also evaluated in terms of usability, e.g., the MeMo
% framework \cite{Moller2006INTERSPEECH}, and more recently, in terms of response
% quality in non-task-oriented neural dialog systems
% \cite{Sordoni2015NAACL,Shang2015ACL,Vinyals2015ICML,Serban2016AAAI,Li2016NAACL,Li2016ACL,luan2017multi,Ghazvininejad2018AAAI},
% where reference-based metrics such as BLEU \cite{BLEU2002} are used.
%\citet{Galley2015ACL} propose $\Delta$BLEU as a discriminative metric for evaluating system responses.
% User engagement has also been studied as a way to evaluate non-task-oriented
% dialog systems \cite{Bohus2009SIGDIAL,Yu2015AAAI,Yu2015SIGDIAL,Yu2016SIGDIAL}

\begin{comment}
Personality awareness to conversational 
agents has been explored in a few studies.
On the agent side,
\citet{mairesse2011controlling} design the language generator in their system to reflect stylistic characteristics of personality types, and \citet{Li2016ACL} add a latent ``persona'' to the neural conversation agent to capture interlocutor characteristics.
On the user side, \citet{mairesse2006automatic} use conversational and linguistic features to infer the user's personality. 
Our system also tries to learn the user's personality, but we use a more direct approach of asking psychologically relevant
questions, in line with \cite{devault2014simsensei,Fung2016ZaraTS}.
\end{comment}


==> chapter_4/_system_data.tex <==
This paper makes use of human-socialbot conversations collected from one
of the Alexa Prize socialbots~\cite{AlexaPrize2017}. 
Hosted on Alexa-enabled devices in the U.S., the system interacts with users 
% using automatic speech recognition and text-to-speech 
by voice using the speech interface provided by the Alexa Prize
platform.
The Alexa Prize platform routes a user's invocation ``\textit{let's chat}'' to a
randomly selected competing socialbot.
The user can terminate the conversation at any time using an explicit
\textit{stop} command.
Afterwards, users can rate the system by responding to the question:
``{\it On a scale of one to five, how much would you like to speak to this socialbot
again?}''

\begin{table}[t]
	\centering
%{\small
	\begin{tabular}{c|c|c|c}
		\hline\hline
		user rating & duration (min) & \# user turns & \# topics \\
		\hline
		3.65 $\pm$ 1.40
		& 4:30 $\pm$ 5:18
		& 22.3 $\pm$ 25.4
		& 8.4 $\pm$ 8.3 \\
		\hline\hline
	\end{tabular}
%}%
	\caption{Statistics of the rated conversations in our dataset, showing there is great variability in user interactions.}.
	\label{tab:data_stats}
\end{table}

%\subsection{Data}
\noindent{\bf Data}:
Our data are collected from a stable system running for one month 
with a consistent dialog policy, but with up-to-date content dynamically added to the back-end.
We only consider conversations with at least three user turns, of which 43\% (68,453) are rated.\footnote{%
	From manual inspection, most short conversations are accidentally started because of incorrect invocation detection; only 11\% of those are rated.
}
Conversation statistics are given in Table\,\ref{tab:data_stats}.
%%MO: Not clear if the 68k is all rated or not, so I put it in the above sentence. Please revise if this is not correct. (I'm also trying to shorten
%our final dataset comprises 68,453 rated conversations.
% Data statistics are shown in Table\,\ref{tab:data_stats}.
% The average number of user turns in the dataset is 19.4, with a standard
% deviation of 24.0.
% The average rating is $3.65$ and the standard deviation is $1.40$.
% The number of topics involved in a conversation varies from 1 to 332, with a
% median of 6 topics per conversation.
We randomly split the data into training, development and test sets with a 3:1:1 ratio.

%\subsection{System}
\noindent{\bf System}:
Alexa Prize socialbots aim to have engaging and coherent conversations with
users about current events.
Following this goal, the system's key design idea is to serve as a
conversational gateway to dynamically updated online content (e.g., news feeds
and discussion forum posts, referred to generally as ``posts'') about various topics.
%We refer to content ``documents'' as ``posts''.
The spoken language understanding (SLU) module uses a multi-dimensional utterance representation by
detecting multiple aspects of user utterances, including intents, questions,
commands, reactions to the post presented by the system, and
topics
mentioned or explicitly requested in the user utterances.
The topic can be either a common noun or noun phrase (e.g., ``milky way''), a proper
noun (e.g., ``Google Earth''), or a general topic (e.g.,
``science'').
Based on manual inspection of 1000 randomly sampled unique user utterances
where the system detects a topic,
% the topic detection precision is 0.99, and the topic extraction accuracy is 0.91.
the false alarm rate is less than 1\%, and the topic extraction error rate is 9\%.
%
Unless users explicitly initiate topics, the system furthers the
conversation by chaining topics together based on entities/topics mentioned in the most recent content
presented to users.
When building a content-informing response, the system 
starts with a grounding phrase based on the SLU output, followed by the post,
%sentence informing 
%the post which 
sometimes rendered as an explicit turn-taking request
(e.g., ``did you know that {\tt \$post}?'').
% \hfang{Re Liz's comment: added an example and corrected the description.}
% and ended with an explicit turn-taking request.
% \maarten{Liz: example would be nice, does ``did you know'' from Fig. \ref{fig:fig1-maarten} count?}

% \noindent{\bf Spoken language understanding (SLU)}:
% \maarten{I think this goes into a little too much detail, we can cut some of it for space}
%\noindent{\bf SLU}:
%For SLU, the 
%The system uses a multi-dimensional utterance representation by
%detecting multiple aspects of user utterances, including intents, questions,
%commands, as well as reactions to the post presented by the system.
%Since most conversations are topic-driven, the SLU actively detects the topics
%mentioned or explicitly requested in the user utterances.
%The topic can be either a common noun or noun phrase (e.g., ``milky way''), a proper
%noun (e.g., a product ``Google Earth''), or some general topic type (e.g.,
%``science'').
%Based on manual inspection of 1000 randomly sampled unique user utterances
%where the system detects a topic,
% the topic detection precision is 0.99, and the topic extraction accuracy is 0.91.
%the false alarm rate is less than 1\%, and the topic extraction error rate is 9\%.
% %\maarten{is 99\% the number of times we detect the right topic when we detect a topic, and 91\% the number of times we correctly detect the right span as a topic?
% Cause if so we don't really need the first number?}
% \hfang{Re Maarten: 99\% is the percentage of times we detect a topic where it is a 
% topic initiation intent.
% 0.91 is the accuracy span extraction accuracy.}

%\subsection{\bf Personality probing}
\noindent{\bf Personality probing}:
%%MO: reworded to get across some idea of why it is only "some"
%For some conversations, 
For conversations from interested users, the system gets noisy\footnote{%
Noise comes from speech recognition and SLU errors,
as well as unreliable user answers.
% Also, the user may not give honest answers.
}
user answers to personality questions adapted from 
the Mini-IPIP questionnaire \cite{donnellan2006mini} through a series of personality 
probing turns.
The answers yield binary scores for each of the five-factor model's personality
traits (openness, conscientiousness, extraversion, agreeableness, neuroticism)
\cite{Costa1992}.
%\citep[openness, conscientiousness, extraversion, agreeableness, neuroticism;][]{costa1992revised}.

% A customized interaction model deployed in the Alexa Skill Kits
% \cite{Kumar2017NIPS} is used as the first-stage dialog-state-independent SLU.
% The system then augments and refines the SLU output using a
% dialog-state-dependent process.
% \maarten{Do we need to mention somewhere that personality affects topic choice?}



==> chapter_5/_dialog_design.tex <==
In the socialbot setting with frequent turn taking, reading the complete article
in one turn is clearly not an option.
An obvious dialog design is to divide the article by sentence and present
individual sentences turn by turn.
To signal the turn taking, a generic question can be appended to the article
sentence, e.g., ``{\it do you want to hear more?}''
If the user shows positive interests, the socialbot can proceed to the next
sentence.  
Otherwise, the socialbot ends the discussion on this article and moves to
another topic.
However, we argue that this is not a satisfying dialog design for four primary
reasons.
First, the original sentence order in the article may not suitable for the turn
by turn interaction, and not every sentence is needed for the conversation.
Second, the information embedded in the generic turn-taking question is too
vague and the user could not easily decide whether they are interested in
knowing it or not.
Third, this dialog design becomes tedious as the conversation progresses since
no other types of social chat content are invovled.
Lastly, this dialog design does not handle targeted information need from the
user, e.g., ``{\it tell me more about Jeff Bezos.}''
With these considerations in mind, we design the dialog of discussing a news
article by formulating five tasks: 
{\bf lead sentence selection},
{\bf follow-up sentence selection},
{\bf introductory clause generation},
{\bf comment retrieval},
and {\bf sentence retrieval}.
They are discussed respectively in
\S\ref{chap5:ssec:lead_sentence}--\ref{chap5:ssec:sentence_retrieval},
followed by a sample conversation in \S\ref{chap5:ssec:sample_conversation}.


\subsection{Lead sentence selection}
\label{chap5:ssec:lead_sentence}
In this thesis, we consider a common way for socialbots to initiate a discussion
on a news article, i.e., inviting the user by informing the headline.
Specifically, we use the following template or its variants, where the
underlined sentence is the title of the news article\footnote{%
	\url{https://tcrn.ch/2R2NBtL}
% \url{https://techcrunch.com/2019/01/22/google-launches-clean-energy-project-in-taiwan-its-first-in-asia/}
}.
\begin{itemize}
	\item {\it I found this news story recently.
		The title was: \uline{Google launches clean energy project in Taiwan,
		its first in Asia.}
		Shall we go through it together?}
\end{center}

If the user agrees to chat about a news article, the socialbot then informs the
lead sentence of the article. 
A good lead sentence should have the following two properties:
First, it should provide the most central information of the article.
Second, it should provide enough new information that is not presented in the
title.
Among the following three sentences from the example news article, the second
sentence is a good lead sentence.
\begin{enumerate}[label={(S\arabic*)},leftmargin=1.2cm]
	\item {\it Google has launched its first clean energy project in Asia.}
	\item {\it The company announced today that it struck a long-term
			agreement to buy the output of a 10-megawatt solar array in Tainan
		City, Taiwan, about 100 km south of its data center in the country.}
	\item {\it Google already has solar and wind projects across North and
		South America, as well as Europe.}
\end{enumerate}
The first sentence (S1), which is actually also the first sentence in the
example news article, is a reasonable summary of the article, but it is clearly
not a good lead sentence given that the socialbot has already told the user the
title.
(S3) is not as good as (S2) since it tells less central information about the
news article. 

\subsection{Follow-up sentence selection}
\label{chap5:ssec:followup_sentence}
Every time the socialbot informs an article sentence to the user, it also makes
a plan in advance about the follow-up sentence chosen from the rest of the
article.
The follow-up sentence will be used to extend the discussion in the next turn if
the user does not request specific information about the article.
Compared with the lead sentence, the choice for follow-up sentences has much more
freedom.
% For example, when selecting the follow-up sentence for the lead sentence, there
% are likely several sentences that are equally central to the news article
% (although less central than the lead sentence).
For example, all sentences below are appropriate follow-up sentences for the lead
sentence (S2).
\begin{enumerate}[resume,label={(S\arabic*)},leftmargin=1.2cm]
	\item {\it The agreement is a collaboration between Google, several Taiwanese
			energy companies and the country's government, which recently revised
			Taiwan's Electricity Act to enable non-utility companies to purchase
		renewable energy directly.}
	\item {\it The solar array will be connected to the same regional power grid
			at Google's Chuanghua County data center, one of two in Asia (the other is
		in Singapore).}
	\item {\it The poles supporting the solar panels will be mounted into
			commercial fishing ponds, an arrangement that Marsden Hanna, Google's
			senior lead of energy and infrastructure, said in a blog post will
			maximize land-use efficiency and respect the local ecology because ``fish
		and solar panels can coexist peacefully.''}
	\item {\it The agreement means Google will get a long-term, fixed electricity
		price for its operations in Taiwan.}
\end{enumerate}

Nevertheless, not every article sentence is suitable as a follow-up sentence, and
the suitability changes depending on the conversation context.
First, similar to the lead sentence, a follow-up sentence should carry enough
information itself.
Moreover, a good follow-up sentence should be understandable given the already
informed sentences.
For example, none of the following sentence is a good follow-up sentence for the
lead sentence (S2).
\begin{enumerate}[resume,label={(S\arabic*)},leftmargin=1.2cm]
	\item {\it Here are the key points from the agreement.}
	\item {\it The revisions are part of Taiwan's new energy policy, aimed at
		phasing out nuclear energy by 2025 and increasing the share of electricity
		generated from renewable sources to 20 percent.}
	\item {\it ``As the Taiwanese government pursues further measures to remove market
			barriers and reduce renewable energy costs, we're hopeful that more
			companies will purchase renewable energy, driving even larger projects
		across Taiwan,'' said Hanna.}
	% \item {\it Google is the first corporate power buyer to take advantage of
	% the revised law.}
	% \item {\it Fishing pond owners will also be compensated for hosting the
	% 	panels.}
\end{enumerate}
(S8) does not bring enough information to the conversation and it cannot be used
as a follow-up sentence in any case.
For (S9) and (S10), it is unclear to the user that what the revisions
refer to and who Hanna is, given only the title and the lead sentence (S2).
However, (S9) can be a good follow-up sentence for (S4), and (S10) is a good
follow-up sentence for (S6).

Lastly, since the news article text needs to be crawled from different online
sources, it is inevitable that the extracted text may contain unwanted
sentences, such as image captions (e.g., ``{\it Image Credits: \dots}''),
advertisements (e.g., ``{\it Watch this video: \dots}''), and external links
(e.g., {\it ``Read more: \dots''}).
The socialbot needs to avoid these sentences in the follow-up sentence selection.


\subsection{Introductory clause generation}
\label{chap5:ssec:introductory_clause}
Although the socialbot has a plan for the follow-up sentence, it does not
directly read the follow-up sentence in the current turn.
Instead, we create an introductory clause that can be seen as a conversational
preview for the follow-up sentence.
For instance, the introductory clause for (S7) can be 
``{\it what the agreement means}'',
which is generated by masking the clausal complement constituent using the word
``{\it what}''.
The socialbot uses the introductory clause in the following question templates
or their variants.
\begin{itemize}
	\item {\it Do you want to know \uline{what the agreement means}?}
	\item {\it Do you know \uline{what the agreement means}?}
\end{itemize}
The question is appended to the current sentence as a turn-taking signal to the
user.
We think it is a better turn-taking question compared to the generic ``{\it do
you want to hear more}'', which becomes repetitive as the conversation
progresses.
The proposed turn-taking question using the introductory clause also provides
necessary information to the user for deciding whether they would like to hear
the follow-up sentence or not.

The use of introductory clause can be viewed as following the maxim of quantity
from Grice's Maxims for conversational communication~\cite{Grice1975}.
In this dialog design, the socialbot avoids being more informative than it
required, i.e., not immediately reading the follow-up sentence.
Nevertheless, the socialbot tries to be as informative as possible, i.e., we
favor the introductory clause than the generic turn-taking question.

\subsection{Comment retrieval}
\label{chap5:ssec:comment_retrieval}
To increase the interactivity, the socialbot can elicit user opinions on the
news article after enough number of article sentences have been informed.
In this case, the socialbot can replace the original turn-taking question
that uses the introductory clause with an open question for opinion-seeking,
such as ``{\it what do you think about this?}''
In the next bot turn, the socialbot can acknowledge the user response and throw
out a relevant comment retrieved from a pool of comments on the news article.
In the socialbot utterance shown below, the underlined sentence is a retrieved
comment. 
\begin{itemize}
	\item {\it Hmm, someone said: \uline{this is a good move}. Do you agree?}
\end{itemize}
While ``{\it hmm}'' and its variants are the default acknowledgement phrase, the
socialbot can replace it based on the actual user response. 
For example, if the user asks ``{\it how about you}'' in their response, the
acknowledgement phrase can be ``{\it I'm not sure, but}''.

The introduction of comments increases the diversity of the interaction and
brings new social chat content that is not included in the article itself.
To return to the mode of informing article sentences, the socialbot can ask
the turn-taking question that uses the introductory clause for the follow-up
sentence, e.g., ``{\it Okay. Anyway, do you want to know \dots?}''


\subsection{Sentence retrieval}
\label{chap5:ssec:sentence_retrieval}
While the four previous tasks described in
\S\ref{chap5:ssec:lead_sentence}--\ref{chap5:ssec:comment_retrieval} are all
about actively providing information to the user,
we also expect the user to request specific information in the article during
the conversation.
A typical such user utterance is ``{\it tell me more about X}'', where X is the
topic the user is interested in.
For handling this intent, the socialbot ignores the original follow-up sentence
and tries to retrieve a sentence about the target topic.
For example, if the topic of interest is ``Google'', then (S3) is a good
sentence to be retrieved.
Note that not all the sentences mentioning the target topic are equally good for
a response to the user's specific request, e.g., neither (S5) nor (S6) is better
than (S3) for the target topic ``Google''.
Discussions on the notion of sentence topics can be found in
\cite[Chatper~4]{Lambrecht1994}.

\begin{table}[t]
	\centering
	\begin{tabular}{c|l|p{13cm}}
		\hline\hline
		{\bf Turn} & {\bf Speaker} & {\bf Utterance} \\ 
		\hline
		1 & User 	& let's chat about recent news \\
		2 & Bot 	& Sure! I found this news story recently. The title was: 
		{\it The billionaires fuelling a space race}.
		Shall we go through it together? \\
		3 & User 	& Sounds good! \\
		4 & Bot 	& Great! The article wrote: 
		{\it Dubbed ``NewSpace'', an increasing number of entrepreneurs are joining in
		the race to create cheap, commercialised space travel.}
		Let's see. 
		Do you know \uline{who are among these entrepreneurs}? \\
		5 & User 	& No, I did not. \\
		6 & Bot 	& {\it Among these entrepreneurs are billionaires Elon Musk, Jeff
			Bezos and Sir Richard Branson, who all made their fortunes in other
		industries.}
		Okay, what do you think about this? \\
		7 & User 	& I think a new space race is beginning. How about you?\\
		8 & Bot 	& I'm not sure, but someone said: \uwave{this probably won't happen
		in their lifetime.} Do you agree? \\
		9 & User 	& That's probably true. \\
		10 & Bot 	& Okay. Anyway, do you want to know \uline{how South
		African-born businessman Elon Musk started SpaceX}? \\
		11 & User & No. Tell me more about Jeff Bezos. \\
		12 & Bot 	& Sure. {\it Amazon founder Jeff Bezos, the world's richest man,
			was one of the first billionaires to jump into the commercial ``space
		race'', starting Blue Origin in 2000.} \\
		\hline\hline
	\end{tabular}
	\caption{A sample multi-turn socialbot conversation for discussing a news
	article.
	The title and retrieved article sentences are shown in {\it the italic font}. 
	Generated introductory clauses are \uline{underlined}.
	The retrieved comment is indicated using \uwave{a wavy underline}.
}
	\label{chap5:tab:sample_conversation}
\end{table}

\subsection{A sample conversation}
\label{chap5:ssec:sample_conversation}

To illustrate the dialog design, Table\,\ref{chap5:tab:sample_conversation}
shows a sample conversation about a news
article\footnote{\url{https://www.bbc.com/news/business-45919650}}.
\begin{itemize}
	\item At turn 2, the bot proposes the news article by informing the title to
		the user.
	\item After the user accepts the proposal at turn 3, the bot reads the lead
		sentence at turn 4.
		The bot ends turn 4 using the question with the introductory clause for the follow-up sentence.
	\item Since the user does not object to hear it at turn 5, the bot proceeds to
		read the follow-up sentence at turn 6.
		The bot ends turn 6 using an opinion-seeking question.
	\item At turn 8, the bot first acknowledges the user question at turn 7 by
		saying ``{\it I'm not sure, but}''.
		Then it reads a comment on the article and asks whether the user agrees.
	\item At turn 10, the bot proposes to return to the follow-up sentence using
		the introductory clause.
	\item At turn 12, the bot retrieves the sentence about Jeff Bezos as
		requested by the user at turn 11.
\end{itemize}


==> chapter_5/_prior_work.r1.tex <==
% This section needs to be revised and expanded.
% \begin{itemize}
% 	\item How other socialbots chat bout news articles?
% 	\item Types of knowledge/document representation and corresponding
% 		construction methods. Driven by the application? Or from the perspective of
% 		unstructured data?
% 		\begin{itemize}
% 			\item Information-Extraction paradigm
% 			\item Narrative Chain
% 			\item QA-based. Also mention question generation \cite{HeilmanPhDThesis}.
% 			\item Vector-space model (typically used for retrieval or classification).
% 		\end{itemize}
% 	\item related work on methods used in this chapter
% \end{itemize}

% \subsection{Socialbot dialog design for discussing news articles}
\hfang{see Mari's notes for reorganization of this section}%
To discuss news articles, existing socialbots have tried to read an
automatically generated summary (usually 4-5 sentences) of the
article~\cite{UWSoundingBoard2017,UTrentoRovingMind2017,HWUAlana2017,HWUAlana2018,EmUEmersonbot2017,EmUIrisBot2018,CMUTartan2018}.
Some other socialbots build question-answering components for news articles
using either heuristic rules~\cite{CMUMagnus2017} or information extraction
methods~\cite{CTUAlquist2017}.
Extending the conversation using relevant Twitter comments on a news article is
used in~\cite{RPIWiseMacaw2017,UCDavisGunrock2018}.

Rather than reading the whole summary in one turn, Alana retrieves a summary
sentence in each turn based on the current user utterance~\cite{HWUAlana2018}.
For narrative stories, Slugbot manually annotated stories
in chunks such that each chunk ends with a natural pausing point~\cite{UCSCSlugbot2018}.
They additionally append tag questions to the end of each chunk to implicitly
discourage the user from asking the bot hard questions they are not capable of
answering.

% Simple strategies have been used to increase interactivity during a multi-turn
% news discussion.
% Rather than reading the whole summary in one turn, Alana retrieves a summary
% sentence in each turn based on the current user utterance~\cite{HWUAlana2018}.
% Gunrock elicits user opinions before presenting relevant Twitter
% comments~\cite{UCDavisGunrock2018}.

\begin{comment}
Our work differs from these work in both dialog design and methods for
automating the socialbot conversation.
In particular, the lead and follow-up sentence selection is different from
summarization since it focus on incrementally informing the article sentences.
The use of introductory clause is also a novel way to engaging users in the
conversation.
While there are prior work on automatically generating factual questions about
news articles using constituency parsing~\cite{HeilmanPhDThesis}, we develop our
generation method primarily based on the recent effors on universal
dependencies.
Although it has been studied in other conversational AI
applications~\cite{Lasecki2013UIST,Huang2015HCC,Huang2016CHI,Swaminathan2017UIST,Huang2017CIC,Huang2018CHI},
the use of crowd-powered method for conversational comment collection is also
new.

A large body of work in story understanding has focused on learning scripts
which represent structured knowledge about stereotypical event sequences
together with their participants.
Chambers and Jurafsky first proposed narrative chains a as a aprtially ordered
set of narrative events that share a common actor called the ``protagnoist''.
A narrative event is a tuple of an event (a verb) and its participants
represented as typed dependencies.
Narrative schemas, script sequent, relgrams.
\end{comment}

% Factual question generation: \cite{HeilmanPhDThesis}



==> chapter_5/_trash.tex <==
\subsection{Narrative chain planning?}
\label{chap5:ssec:narrative_chain}
The first type of knowledge the socialbot needs to have is the .


In order to \dots, the socialbot needs to understand the story.
A large body of work in story understanding has focused on learning scripts
which represent structured knowledge about stereotypical event sequences
together with their participants.
Chambers and Jurafsky first proposed narrative chains a as a aprtially ordered
set of narrative events that share a common actor called the ``protagnoist''.
A narrative event is a tuple of an event (a verb) and its participants
represented as typed dependencies.
Narrative schemas, script sequent, relgrams.


In a news article, not all sentence are equally informative.

We first identify a subset of sentences from the article that satisfying the
following criteria.
1) The sentence provides new information ?
2) The sentence itself forms a natural end of an information chunk.
Multi-sentence quotes are excluded.
3) The sentence should not be too short or other.
4) The sentence should not be image/video captions, etc.

produce a chain of sentences from the article that capture the 

identify a set of sentences from the article which are 
going to be
informed by the socialbot during the course of the conversation.
We use a 
We call the sequence as the {\bf narrative chain} for the socialbot conversation.

Each information unit will be presented in a socialbot turn. 
In this chapter, we focus on using a sentence as an information unit.

While a narrative chain can be extended to multiple sentences and multiple
paths, we leave them as future work.

greedy next sentence selection.

Most news article follow an inverse pyramid structure \cite{}.

TBD

Other considerations.
First, sentence filtering. Not good for text-to-speech synthesis.
Short sentences.


For example, for the sentence ``{\it Party chairman Gilberto Hinojosa said in a
statement that Texas Republican government blamed voters and did nothing}'', we
can generate an introductory phrase ``{\it what Party chairman Gilberto Hinojosa
said in a statement}'' by masking the clausal complement constituent using the
word ``{\it what}''.
The introductory phrase will then be used by the socialbot in a question form
such as ``{\it do you want to know what Party chairman Gilberto Hinojosa said in
a statement}''.

The introductory phrase will then be used by the socialbot in a question form
such as 
to engage the user in the conversation.


mentally prepared for what happens next.

There are other types of introductory phrase, depending on the semantic
constituents being masked.

``{\it more about Party chairman Gilberto Hinojosa}''
by, or 

From the linguistic perspective,
the introductory phrase can be viewed as the theme of the sentence and 
topic-comment theory,
information structure theory.
Intonation.

can be used for proactively engage the user in the discussion

satisfying the user's information need,
engaging seed.

vs.\ summarization:
incremental/sequential/redundant.
every sentence.

\subsection{Content planning}
2) summarization, narrative chain;
3) Slugbot v2 \cite{UCSCSlugbot2018}: narrative stories, chunking the stories
(annotation), append tag questions to the end of each chunk to ``implicitly
discourage the user from asking us hard questions we are not capable of
answering.'';

\subsection{Question generation}
Factual question generation: \cite{HeilmanPhDThesis}


{\bf Future Work}:
deeper recursive analysis of clausal complements, 
e.g., deeper dobj.



\section{Conclusion and Future Work}
If we cannot find any sentence that is about the requested topic, the socialbot
apologizes and suggests another sentence using the introductory phrase

In this thesis, we focus on handling the user's information need on a specific
topic in the article, which can be fulfilled within the system's language
understanding capacity.
Other types of user information need including complex requests (e.g., ``{\it
tell me what kinds of aid they received}'') and question answering (e.g., ``{\it
why did this happen}'')
are beyond the scope of this thesis.
We currently use the generic sentence ``{\it let's see if the article tells
us}'' or its variants to deflect such requests, appended with the follow-up
sentence.




\begin{comment}
using \textlangle node,
relation, node\textrangle\ triplets.
We currently consider three core node types:
\textsf{title}, \textsf{sentence}, and \textsf{entity}.
For these nodes, we define a set of relations (\textsf{hasFollowupSentence},
\textsf{isFollowupSentenceOf}, \textsf{hasTopic}, \textsf{isTopicOf}),
resulting the following types of triplets. 
\begin{itemize}
	\item \textlangle \textsf{title}, \textsf{hasFollowupSentence}, \textsf{sentence}\textrangle
	\item \textlangle \textsf{sentence}, \textsf{isFollowupSentenceOf}, \textsf{title}\textrangle
	\item \textlangle \textsf{sentence}, \textsf{hasFollowupSentence}, \textsf{sentence}\textrangle
	\item \textlangle \textsf{sentence}, \textsf{isFollowupSentenceOf}, \textsf{sentence}\textrangle
	\item \textlangle \textsf{sentence}, \textsf{hasTopic}, \textsf{entity}\textrangle
	\item \textlangle \textsf{entity}, \textsf{isTopicOf}, \textsf{sentence}\textrangle
\end{itemize}


% Shift the burden of reasoning to offline, so that the dialog management can
% focus on dialog control, less computation on reasoning.

% Having a summary \dots does not necessarily alleviate this issue.

% Our goal is to develop a knowledge/ontology representation that is ready to use by
% socialbots for carrying out extended conversations on news articles.

The basic representation which can be immediately constructed is to represent
the article by individual sentences.
In the socialbot setting with frequent turn taking, reading the complete article
in one turn is clearly not an option.
A simple dialog strategy is to divide the article by sentence and present
individual sentences turn by turn.
To signal turn taking, a generic question can be appended to the article
sentence, e.g., ``{\it do you want to hear more?}''
If the user shows positive interest, the socialbot can proceed to the next
sentence.  
Otherwise, the socialbot ends the discussion on this article and moves to
another topic.


\begin{table}[t]
	\centering
	\begin{tabular}{l|p{12.6cm}}
		\hline\hline
		{\bf Attribute}  & {\bf Description} \\
		\hline
		Index & The index (position) of the sentence in the article. \\
		Text & The sentence text. \\
		Constituents &  The semantic constituents of the sentence, including the
		subject, object, etc. \\
		Introductory Clause & A clause that is used to present a
		conversational preview of the sentence. \\
		% Next Sentence & The index of the next sentence in the default narrative
		% plan.\\
		\hline\hline
	\end{tabular}
	\caption{The knowledge representation of a sentence in a news article.}
	\label{chap5:tab:knowledge_representation}
\end{table}
To prepare for discussing a news article, we build a knowledge representation
for individual article sentences.
The knowledge representation consists of attributes shown in
Table\,\ref{chap5:tab:knowledge_representation}.
Both the index and the text are basic attributes that are straightforward to
obtain.
The semantic constituents are obtained from the dependency parsing analysis of
the sentence, including the predicate, subject, object, and etc.
These constituents are used for two purposes:
1)~retrieve sentences when the user requests information about a specific entity,
and 2)~automatically build the introductory clause.

\begin{table}[t]
	\centering
	\begin{tabular}{l|l}
		\hline\hline
		{\bf Attribute}  & {\bf Description} \\
		\hline
		Subject Entity &  The subject entity of the sentence. \\
		Introductory Clause & A clause for introducing the sentence during the
		conversation. \\
		Follow-up Sentence & The pre-selected follow-up sentence for the
		conversation. \\
		Comment & The opinion statement in respond to the sentence. \\
		\hline\hline
	\end{tabular}
	\caption{Core attributes in the sentence representation.}
	\label{chap5:tab:sentence_representation}
\end{table}

\end{comment}

\subsection{Question generation} 
\label{chap5:ssec:algo_iclause_generation}

\hfang{major revision on this subsection}%
We propose a method using the dependency parsing results to automatically
generate questions for the individual sentences in the article.
Consider the example sentence in
Fig.\,\ref{chap5:fig:sample_sentence_dependency}, 
a question node can be generated to represent the question ``{\it what did Party
chairman Gilberto Hinojosa say in a statement}''.
The question node is represented using a tuple of sentence constituents
\textlangle what, Party chairman Gilberto Hinojosa, said, in a statement\textrangle,
where ``said'' is the predicate of the sentence, ``Party chairman Gilberto
Hinojosa'' is the subject (\textsf{nsubj}) of the predicate, ``in a statement'' is
the nominal modifier (\textsf{nmod}) of the predicate, and ``what'' is the
question type corresponding to the clausal complement (\textsf{ccomp})
of the predicate.

\begin{table}[t]
	\centering
	\begin{tabular}{l|l|l}
		\hline\hline
		{\bf Constituent} & {\bf Dependency Path} & {\bf Description} \\
		\hline
		%%%%%%%%%%%%%%%%%%
		V & \textsf{root} & predicate of the sentence \\
		\hline
		%%%%%%%%%%%%%%%%%%
		% & /\textsf{root}/ & dependents of the predicate \\
		S & \textsf{root}/(\textsf{nsubj}\textbar\textsf{nsubjpass}) 
		& nominal subject or passive nominal subject of V \\
		%
		O\textsubscript{i}  & \textsf{root}/\textsf{iobj} 
		& indirect object of V \\
		%
		O\textsubscript{d} 	& \textsf{root}/\textsf{dobj} 
		& direct object of V \\
		%
		O\textsubscript{ccomp} & \textsf{root}/\textsf{ccomp}
		& clausal complement of V functioning as an object \\
		%
		% it is an adverb or adverbial phrase
		% A\textsubscript{advmod} & \textsf{root}/\textsf{advmod}
		% & non-clausal adverbial modifier of V \\
		%
		A\textsubscript{advcl} & \textsf{root}/\textsf{advcl}
		& adverbial clause modifier of V \\
		%
		A\textsubscript{nmod} & \textsf{root}/\textsf{nmod}
		& nominal modifier of V functioning as an adverbial \\
		%
		A\textsubscript{nmod-tmod} & \textsf{root}/\textsf{nmod-tmod}
		& temporal modifier of V \\
		D & \textsf{root}/\textsf{dep} & 
		unspecified dependency of V \\
		%
		C\textsubscript{xcomp} & \textsf{root}/\textsf{xcomp}
		& open clausal complement of V \\
		N 	& \textsf{root}/\textsf{neg} & negation modifier of V \\	
		\hline
		%%%%%%%%%%%%%%%%%%
		% & /\textsf{root}/\textsf{xcomp}/ & 
		% dependents of the open clausal complement's root \\
		X\textsubscript{mark} & \textsf{root}/\textsf{xcomp}/\textsf{mark} 
		& marker of C\textsubscript{xcomp} \\
		% X\textsubscript{subj} & \tabitem \textsf{nsubj}, \textsf{nsubjpass} 
		% & \tabitem nominal subject or passive nominal subject \\
		X\textsubscript{dobj} & \textsf{root}/\textsf{xcomp}/\textsf{dobj} 
		& direct object of C\textsubscript{xcomp} \\
		X\textsubscript{ccomp} & \textsf{root}/\textsf{xcomp}/\textsf{ccomp} 
		& clausal complement of C\textsubscript{xcomp} \\
		\hline\hline
	\end{tabular}
	\caption{Core constituents and corresponding dependency paths.}
	\label{chap5:tab:clause_constituents}
\end{table}

To generate question nodes, we first use the dependency parsing outcome to
extract sentence constituents.
Specifically, the RDFLib\footnote{\url{https://rdflib.readthedocs.io/}} is used
to convert the dependency parsing results to a semantic graph according to the
resource description framework (RDF), where the edge from the governor node to
the dependent node is labeled by the corresponding dependency relation.
The SPARQL query language\footnote{\url{https://www.w3.org/TR/sparql11-query}}
is used to extract the head word of the constituents.
The core constituents and corresponding dependency paths are summarized in
Table\,\ref{chap5:tab:clause_constituents}.
The dependency paths originated from the notional sentence root are described
using the property path syntax of the SPARQL query language.
Note that not every constituents in Table\,\ref{chap5:tab:clause_constituents}
appears in a sentence, and some constituents (e.g., S, O\textsubscript{d},
A\textsubscript{nmod}) may appear multiple times.
The only exception is the predicate V, which always appears exactly once in a
sentence.\footnote{\url{http://universaldependencies.org/docsv1/u/dep/root.html}}

\begin{table}[t]
	\centering
	\begin{tabular}{l|l}
		\hline\hline
		{\bf Dependency Path} & {\bf Question Types}  \\
		\hline
		\textsf{root}/(\textsf{nsubj}\textbar\textsf{nsubjpass})/\textsf{nummod} & how many \\
		\textsf{root}/\textsf{ccomp} 				& what \\
		\textsf{root}/\textsf{dobj} 				& what, who \\
		\textsf{root}/\textsf{nmod-tmod} 		& when \\
		\textsf{root}/\textsf{nmod} 				& how, what, when, where, why \\
		\textsf{root}/\textsf{advcl} 				& how, what, when, why  \\
		\textsf{root}/\textsf{xcomp}/\textsf{ccomp} 		& what \\
		\textsf{root}/\textsf{xcomp}/\textsf{dobj} 			& what, who \\
		\textsf{root}/\textsf{xcomp}/\textsf{nmod}  		& how, what, when, where, why \\
		% noun
		\textsf{root}/\textsf{xcomp}  			& POS what \\
		% adj
		\textsf{root}/\textsf{xcomp}  			& how \\
		\hline
		% only for vpred
		\textsf{root}/\textsf{dep} 		& what \\
		\textsf{root}/\textsf{neg} 		& whether \\
		% only for npred
		\textsf{root} 								& what \\
		\hline
	\end{tabular}
	\caption{Detected \texttt{question} edges with corresponding question
	type and arguments.
	`?' indicates zero or one such constituent.
		`*' indicates zero or more such constituents, ordered by their original
		positions in the sentence.
	}
	\label{chap5:tab:question_edges}
\end{table}

\begin{table}[t]
	\centering
	\begin{tabular}{l|l|l}
		\hline\hline
		{\bf Answer Constituent} & {\bf Question Types} 
		& {\bf Question Constituents} \\
		\hline
		S\textsubscript{nummod} & how many
		& & \\
		O\textsubscript{ccomp} & what
		& S V O\textsubscript{i}? O\textsubscript{d}? A\textsubscript{nmod}* \\
		% 
		D & what
		& S V O\textsubscript{i}? O\textsubscript{d}? A\textsubscript{nmod}* \\
		% 
		O\textsubscript{dobj} & what, who
		& S V O\textsubscript{i}? A\textsubscript{nmod}* \\
		%
		A\textsubscript{nmod-tmod} & when
		& S V O\textsubscript{i}? A\textsubscript{nmod}* \\
		%
		\hline
		A\textsubscript{advcl} & & \\ 
		\hline
		% 
		A\textsubscript{nmod}
		& V O\textsubscript{d}? \\
		\hline
		%
		X\textsubscript{ccomp} & what
		& S V O\textsubscript{i}? O\textsubscript{d}? A\textsubscript{nmod}*
		X\textsubscript{mark}* C\textsubscript{xcomp} \\
		%
		X\textsubscript{dobj} & what, who
		& S V O\textsubscript{i}? O\textsubscript{d}? A\textsubscript{nmod}*
		X\textsubscript{mark}* C\textsubscript{xcomp} \\
		%
		X\textsubscript{nmod}: VPRED & & \\
		%
		C\textsubscript{xcomp}: NOUN & what 
		& S V O\textsubscript{i}? O\textsubscript{d}? A\textsubscript{nmod}*
		X\textsubscript{dep,mark,cop}* \\
		%
		C\textsubscript{xcomp}: ADJ & how
		& S V O\textsubscript{i}? O\textsubscript{d}? A\textsubscript{nmod}*
		X\textsubscript{dep,mark,cop}* \\
		\hline\hline
	\end{tabular}
	\caption{Detected \texttt{question} edges with corresponding question
	type and arguments.
	`?' indicates zero or one such constituent.
		`*' indicates zero or more such constituents, ordered by their original
		positions in the sentence.
	}
	\label{chap5:tab:question_edges}
\end{table}

Each \texttt{question} edge is labeled by a question type and an argument
sequence.
In this work, we identify several \texttt{question} edges as shown
in Table\,\ref{chap5:tab:question_edges} based on the constituents derived at
step~2.
Since a \texttt{question} edge connects a sentence node and its subject entity
node, S is omitted in the table.
The constituent in the argument sequence is associated with its textual
representation in its entirety by extracting corresponding dependents of the
constituent.
To generate the introductory clause for the \texttt{question} edge, the
socialbot can simply concatenate the question type attribute, the subject
entity, and the argument sequence.\hfang{ask Mari: move this to 5.4.2?}

% \textlangle what-O\textsubscript{ccomp}, said-V\textrangle\
% can be created where O\textsubscript{ccomp} means the clausal complement
% constituent which acts as an object and V refers to the predicate. 
% \hfang{add a table with examples of constituents and
% 	dependencies and question edge identified for the sentence in the example.}
% The corresponding introductory clause for the \texttt{question} edge is 
% ``{\it what Party chairman Gilberto Hinojosa said}''.

% question type, including what, who, why, where, when, whether, how, how many.

% Similar to a proposition defined in the ClausIE, an introductory clause consists
% of a subject (``{\it Party chairman Gilberto Hinojosa}''), 
% a relation (``{\it said}''), 
% one or more arguments (``{\it in a statement}'') being exposed,
% and one argument (``{\it that Texas Republican government blamed voters and did
% nothing}'') being masked by an interrogative word (``{\it what}'').

\begin{comment}
For each sentence, the proposed method carries out the following steps:
\begin{enumerate}
	\item Obtain the dependency parsing and part-of-speech (POS) tagging
		predictions.
	\item Derive the core constituents for \texttt{question} edges using the
		parsing outcome.
	\item Generate possible \texttt{question} edges for the sentence by masking
		its constituents using pre-defined templates.
\end{enumerate}

\begin{table}[t]
	\centering
	\begin{tabular}{l|l|l}
		\hline\hline
		{\bf Constituent} & {\bf Dependency Path} & {\bf Description} \\
		\hline
		%%%%%%%%%%%%%%%%%%
		V & \textsf{root} & predicate of the sentence \\
		\hline
		%%%%%%%%%%%%%%%%%%
		% & /\textsf{root}/ & dependents of the predicate \\
		S & \textsf{root}/(\textsf{nsubj}\textbar\textsf{nsubjpass}) 
		& nominal subject or passive nominal subject of V \\
		%
		O\textsubscript{i}  & \textsf{root}/\textsf{iobj} 
		& indirect object of V \\
		%
		O\textsubscript{d} 	& \textsf{root}/\textsf{dobj} 
		& direct object of V \\
		%
		O\textsubscript{ccomp} & \textsf{root}/\textsf{ccomp}
		& clausal complement of V functioning as an object \\
		%
		% it is an adverb or adverbial phrase
		% A\textsubscript{advmod} & \textsf{root}/\textsf{advmod}
		% & non-clausal adverbial modifier of V \\
		%
		A\textsubscript{advcl} & \textsf{root}/\textsf{advcl}
		& adverbial clause modifier of V \\
		%
		A\textsubscript{nmod} & \textsf{root}/\textsf{nmod}
		& nominal modifier of V functioning as an adverbial \\
		%
		%
		A\textsubscript{nmod_tmod} & \textsf{root}/\textsf{nmod_tmod}
		& temporal modifier of V functioning as an adverbial \\
		D & \textsf{root}/\textsf{dep} & 
		unspecified dependency of V \\
		%
		C\textsubscript{xcomp} & \textsf{root}/\textsf{xcomp}
		& open clausal complement of V \\
		\hline
		%%%%%%%%%%%%%%%%%%
		% & /\textsf{root}/\textsf{xcomp}/ & 
		% dependents of the open clausal complement's root \\
		X\textsubscript{mark} & \textsf{root}/\textsf{xcomp}/\textsf{mark} 
		& marker of C\textsubscript{xcomp} \\
		% X\textsubscript{subj} & \tabitem \textsf{nsubj}, \textsf{nsubjpass} 
		% & \tabitem nominal subject or passive nominal subject \\
		X\textsubscript{dobj} & \textsf{root}/\textsf{xcomp}/\textsf{dobj} 
		& direct object of C\textsubscript{xcomp} \\
		X\textsubscript{ccomp} & \textsf{root}/\textsf{xcomp}/\textsf{ccomp} 
		& clausal complement of C\textsubscript{xcomp} \\
		\hline\hline
	\end{tabular}
	\caption{Core constituents and corresponding dependency paths.}
	\label{chap5:tab:clause_constituents}
\end{table}

{\bf Step 1 -- Dependency Parsing and POS Tagging}:
We obtain the dependency parsing and POS tagging results from the Stanford CoreNLP toolkit
(v3.9.1)~\cite{CoreNLP}.
An example sentence is shown in
Fig.\,\ref{chap5:fig:sample_sentence_dependency}. 
The toolkit uses a neural transition-based dependency parsing
model~\cite{Chen2014EMNLP} and follows the universal dependency relations\footnote{%
	\url{http://universaldependencies.org/docsv1}
}
defined in~\cite{UniversalDependenciesV1}.
The proposed method for introductory clause generation is based on these
universal dependency relations.
The POS tagger uses the Penn Treebank tagset~\cite{PennTreebank}.
We convert the tags to universal POS tags using the map defined
in~\cite{Petrov2012LREC}.

{\bf Step 2 -- From Dependencies to Constituents}:
Core constituents for \texttt{question} edges are identified using the
dependency relations.
First, the RDFLib\footnote{\url{https://rdflib.readthedocs.io/}} is used to
convert the dependency parsing results to a semantic graph according to the
resource description framework (RDF), where the edge from the governor node to
the dependent node is labeled by the corresponding dependency relation.
Then, the SPARQL query
language\footnote{\url{https://www.w3.org/TR/sparql11-query}} is used to extract the
head word of the constituents.
The identified core constituents and corresponding dependency paths are
summarized in Table\,\ref{chap5:tab:clause_constituents}.
The dependency paths originated from the notional sentence root are described
using the property path syntax of the SPARQL query language.
Note that not every constituents in Table\,\ref{chap5:tab:clause_constituents}
appears in a sentence, and some constituents (e.g., S, O\textsubscript{d},
A\textsubscript{nmod}) may appear multiple times.
The only exception is the predicate V, which always appears exactly once in a
sentence.\footnote{\url{http://universaldependencies.org/docsv1/u/dep/root.html}}

\begin{table}[t]
	\centering
	\begin{tabular}{l|l}
		\hline\hline
		% \multicolumn{2}{c|}{\bf Type} & {\bf Arguments} \\
		{\bf Type} & {\bf Argument Sequence} \\
		\hline
		% 
		% if has ccomp, ignore
		% if dobj too simple and there is nmod, nmod overwrites it
		% if has advcl and no other constituents? 
		% if too complex
		what-O\textsubscript{dobj}
		& V O\textsubscript{i}? A\textsubscript{nmod}* \\
		%
		what-O\textsubscript{ccomp}
		& V O\textsubscript{d}? A\textsubscript{nmod}* \\
		% 
		how-A\textsubscript{advcl}
		& V O\textsubscript{d}? A\textsubscript{nmod}* \\
		% & why S V O\textsubscript{d} \\
		% 
		how-A\textsubscript{nmod}
		& V O\textsubscript{d}? \\
		%
		what-D
		& V A\textsubscript{nmod}* \\
		%
		what-X\textsubscript{dobj}
		& V O\textsubscript{d}? A\textsubscript{nmod}* X\textsubscript{mark}*
		C\textsubscript{xcomp} \\
		%
		what-X\textsubscript{ccomp}
		& V O\textsubscript{d}? A\textsubscript{nmod}* X\textsubscript{mark}*
		C\textsubscript{xcomp} \\
		\hline\hline
	\end{tabular}
	\caption{Detected \texttt{question} edges with corresponding question
	type and arguments.
	`?' indicates zero or one such constituent.
		`*' indicates zero or more such constituents, ordered by their original
		positions in the sentence.
	}
	\label{chap5:tab:question_edges}
\end{table}

\begin{comment}
\begin{table}[t]
	\centering
	\begin{tabular}{l|c|l}
		\hline\hline
		{\bf Constituent} & {\bf Universal POS} & {\bf Dependency Path} \\
		\hline
		V & VERB & 
		\textsf{root}/(\textsf{compound}\textbar\textsf{compound-prt})
		\\
		S & NOUN &
		\textsf{root}/(\textsf{nsubj}\textbar\textsf{nsubjpass})/(\textsf{nmod}\textbar\dots)+
		\\
		\hline\hline
	\end{tabular}
	\caption{Textual representation of constituents.}
	\label{chap5:tab:constituent_realization}
\end{table}
\end{comment}

{\bf Step 3 -- From Constituents to Question Edges}:
Each \texttt{question} edge is labeled by a question type and an argument
sequence.
In this work, we identify several \texttt{question} edges as shown
in Table\,\ref{chap5:tab:question_edges} based on the constituents derived at
step~2.
Since a \texttt{question} edge connects a sentence node and its subject entity
node, S is omitted in the table.
The constituent in the argument sequence is associated with its textual
representation in its entirety by extracting corresponding dependents of the
constituent.
To generate the introductory clause for the \texttt{question} edge, the
socialbot can simply concatenate the question type attribute, the subject
entity, and the argument sequence.\hfang{ask Mari: move this to 5.4.2?}
\end{comment}
% We use a decision tree to decide the introductory to use when there are multiple
% choices.\hfang{I intentionally make this paragraph vague since I haven't
% finalized the process.}
% Table\,\ref{chap5:tab:constituent_realization} summarizes the dependency paths
% for extracting the dependents of the clause constituent, depending on their
% universal POS tags.
% For constituents with an unusual POS tag, we simply do not generate the clause. 

\begin{comment}
\begin{table}[t]
	\centering
	\begin{tabular}{l|c|l}
		\hline\hline
		{\bf Constituent} & {\bf Universal POS} & {\bf Dependency Path} \\
		\hline
		V & !NOUN &
		\textsf{root}/(\textsf{neg}\textbar\textsf{cc}\textbar\textsf{conj}) \\
		S & - &
		\textsf{root}/(\textsf{nsubj}\textbar\textsf{nsubjpass})/(\textsf{neg}\textbar\textsf{cc-preconj})
		\\
		\hline\hline
	\end{tabular}
	\caption{Negative patterns.}
	\label{chap5:tab:negative_patterns}
\end{table}
\end{comment}


{\bf Special Cases}:
We do not generate the \texttt{question} edge if the predicate V is not a
verb or has any of the following three types of dependents: negation modifier
(\textsf{neg}), coordinating conjunction (\textsf{cc}), and conjunction
(\textsf{conj}). 
These cases complicate the templates for questions and introductory clauses. 
For example, when A\textsubscript{nmod} attaches to a noun predicate,
it functions as an attribute or genitive complement rather than an adverbial,
and thus, ``how'' is not the right question type.
Second, we do not generate the \texttt{question} edge if there is more than one
subject or the subject S has a negation (\textsf{neg}) dependent or a
preconjunct (\textsf{cc:preconj}) dependent (e.g., ``{\it either}'', 
``{\it both}'', ``{\it neither}'').
Clausal subjects (\textsf{csubj} and \textsf{csubjpass}) are ignored, which are
rare (around 1\% sentences) in the collected data.
A different process needs to be developed to handle these cases, which is beyond
the scope of this work.

\begin{comment}
The following methods are compared for our experiments.
\begin{itemize}
	\item {\bf SentenceDistance}: This method simply ranks the candidate sentence
		based on their distance in terms of position in the article from the last
		sentence in the storytelling chain.
		Since we only consider sentences after the last sentence in the chain,
		this method essentially ranks sentences based on their original position in
		the article. 
		In other words, a sentence appeared earlier in the article gets a better
		ranking.
	\item {\bf TextRank}: This method uses the TextRank
		algorithm~\cite{Mihalcea2004EMNLP,Barrios2016arXiv} implemented in
		Gensim~\cite{Gensim}.
		The algorithm is originally proposed for unsupervised extractive
		summarization by scoring sentences based on their centrality in the article.
		We use the algorithm to score all sentences in the article, and then rank
		the candidate sentences in the annotation unit.
	\item {\bf BERT without Context + LogisticRegression}:
		This method uses pre-trained BERT to derive an embedding for the candidate
		sentence without using the context sentences $(x_1, \dots, x_l)$.
		The logistic regression model uses the sentence embedding as the input
		feature for binary classification in the same as the model described in
		\S\ref{chap5:ssec:model_storytelling_chain}.
	\item {\bf BERT with Context + LogisticRegression}:
		This is the method describes in \S\ref{chap5:ssec:model_storytelling_chain},
		which uses BERT to derive embeddings for pairs of the candidate sentence and
		its context sentences. 
\end{itemize}

Test set results are shown in Table\,\ref{chap5:tab:exp_sentence_selection}.
We report results on two subsets, i.e., $l=1$ and $l=2$.
First, it can be observed that the SentenceOrder baseline performs the worst.
The accuracy values indicate that only in 54.7\% cases the immediate next sentence
in the article is good as a follow-up sentence for the storytelling chain when
$l=1$, since it is common that the first few sentences in the article provides
redundant information when the title is already given.
For $l=2$, the number is slightly higher, i.e., 62.3\%, but there are still
plenty of cases where the next sentence in the article is not a good candidate.
Second, the unsupervised summarization algorithm TextRank performs better than
SentenceOrder, indicating that the sentence importance/centrality is useful for
building the storytelling chain.
For supervised logistic regression models, it can be seen that using the
candidate sentence alone without context sentences already performs
significantly better than the SentenceOrder baseline.
Nevertheless, it does not outperform the TextRank method.
Taking into account context sentences can boost the performance significantly
and achieves the best results among all compared methods.
Interestingly, 

since it does not have
access to other sentences

The supervised models 

It can be seen that the logistic regression models consistently outperform
baseline methods.
% The gain is more significant for $l=1$ than $l=2$.


\begin{table}[t]
	\centering
	\begin{tabular}{l|c|c}
		\hline\hline
		{\bf Model} 				& $l=1$ & $l=2$ \\
		\hline
		SentenceDistance 		& 54.7 & 62.3 \\
		TextRank 						& 63.2 & 71.9 \\
		\hline
		BERT without Context    			& 62.1  & 69.3 \\
		BERT with Context    					& 68.4 	& 73.7 \\
		BERT with Context + TextRank 	& 68.4 	& 75.4 \\
		\hline\hline
	\end{tabular}
	\caption{Test set performance of different methods for creating storytelling
		chains.}
	\label{chap5:tab:exp_sentence_selection}
\end{table}
\end{comment}



==> chapter_6/_future_work.tex <==
Being a new type of conversational AI, there are plenty of interesting
directions for future research on socialbots.
In this work, we have formulated the dialog flow of a miniskill as a finite
state machine and have manually specified the transitions between states due to 
the fact that the socialbot research is in an early stage that makes
it difficult to create a corpus for learning a statistical dialog manager.
Often challenges to use of a statistical DM are that 1) there is no consensus on
the inventory of state, and 2) new capabilities are frequently added to a
socialbot that interacts with real users.
The proposed hierarchical DM framework can alleviate some of these issues as it
allows the system to upgrade a miniskill dialog manager to a statistical version
with
minimal impacts on other components of the socialbot.
The proposed multi-level reward functions are also useful for learning the
dialog policy in this scenario.\hfang{Say more about the reward functions}

\hfang{The rest part is not very well organized. I'll improve it later on.}
The proposed document representation can also be applied to other types of
documents beyond news articles, such as Wikipedia pages, legal documents, etc.
% find the motivations of storytelling workshop
Data-driven models can also be developed for the question generation, which
could be an interesting task for natural language generation research.
% For example, we can envision a sequence-to-sequence neural model that takes the
% input of the sentence and its dependency parsing representation.

%%%%%%%%%%%%%%%%%%%%%%%
% use of user ratings?
% reinforcement learning: long-term reward
% user modeling
%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
In terms of the system development, more natural language processing tools need
to be developed for language understanding, especially for handling ellipsis and
anaphora resolution which are frequently observed in socialbot conversations.
\end{comment}
%%%% extended entities

Existing large-scale public knowledge bases are predominately focused on proper
entities (e.g., Freebase \cite{Freebase2008}, DBpedia \cite{DBpedia2015}}) and
common-sense knowledge (e.g., ConceptNet \cite{ConceptNet2004,ConceptNet2017}).
While these types of knowledge are useful for retrieving factual information and
reasoning, we have shown that social chat content also plays an important role
in socialbots.
Social media platforms have been used to collect social chat content.
However, they inevitably contain useless, boring, inappropriate, and even wrong
information.
A family-friendly socialbot should avoid mentioning content about sex, violence,
racism, hate speech, etc.
Therefore, we need to be extremely careful about the social appropriateness of
the content.
It is useful to develop methods that automatically identify inappropriate
content. 
This issue has attracted a lot of interest recently, and there is a rapidly
growing body of work on detecting hate speech and offensive content.
However, the broader question of identifying socially appropriate content is not
yet addressed.
% one can measure the quality of the content from different aspects such as
% informativeness, authority, popularity, novelty, etc.
% Using multiple measures may be useful for different types of content and/or for
% serving different types of users.

Challenges of a conversational interface have prevented recommender systems from
the adoption of natural language interactions, leaving the conversational
recommendation as untapped potential.
We anticipate that the socialbot can promote the integration of dialog systems
and recommender systems.
Furthermore, while this thesis has focused on the socialbot that talks about
recent events and popular topics, we envision socialbots can have a broad range
of applications beyond entertainment, such as language learning and information
kiosk.

% In summary, conversational AI has long been an active research area and will
% contiune to be an exciting area attracting more research interests.


==> chapter_6/_trash.tex <==
% Nevertheless, the information acquisition process in most existing information
% retrieval and recommender systems lacks the interactive nature of human social
% behaviors.
% For example, users may not be fully aware of their preferences or prefer to hold
% their decisions until they have interacted with the system for a while and
% roughly understand the range of alternatives.

% MOVE TO related work
Specifically, the novelty/serendipity, which measures whether a recommendation
is a novel possibility for a user, has been brought to attention in the
recommender system research \cite{Herlocker2004}.

% PARTIALLY MOVED TO Challenges
There is growing interest in moving from traditional limited-domain
conversational AI systems towards open-domain systems.
A domain can mean a simple task (e.g., setting alarms), a complex task
(e.g., travel planning) involving multiple sub-tasks, a specific topic (e.g.,
sports), a specific application (e.g., psychology counselling), and etc.
Sometimes, a domain is described by the underlying ontology of the system's
knowledge base (KB) backend.
The coverage of domain is bound by the KB\dots
In recent years, with easier access to online information and advances in
language processing technologies, enriching the KB at scale
becomes possible.
With a wide coverage of domains, the system can provide more comprehensive user
experiences and also maintain a high level of user curiosity in exploring the
system.
However, carrying out open-domain conversations is non-trivial and raises
challenges such as coherent domain chaining and smooth domain transitions.
Interpretation, decision logic, presentation.
\cite{Young2010SPM}

\begin{itemize}
	\item User utterance representation.
		``{\it In spoken dialog systems, the mode widespread models of SLU are based on the
			identification of slots (entities) within on or more frames (frame-slot
		semantics) defined by the application domain.}''
		Ontology as a domain model in order to exploit not only knowledge about the
		properties of individual concepts, but also their relations, expressed in
		terms of classical semantic relations.
		Ontology design.
	\item Speech act vocabulary. 
		Each speech act corresponds to a parameterised templates with several
		different realisation.
\end{itemize}

Although they are requested by the DM policy making, they can be relatively
developed independently. 

A collection of policies.
understanding policy refines.


Input: 
1) current user utterance,
2) context variables:
2.1) user profile
2.2) content history

User profile representation.
Mental states.

Output:
1) Speech Acts

Utterance-level ontology.
User profile representation.

When receiving the uesr utterance

The NLU produces a representation of the current event by analyzing the user’s
speech given the current dia- log state (§2.1). Then, based on this
representation,
the DM executes the dialog policy and decides the
next dialog state (§2.2). Finally, the NLG uses the
content selected by the DM to build the response
(§2.3), which is returned to the user and stored as
context in the DM. During the conversation, the
DM also communicates with a knowledge graph
that is stored in the back-end and updated daily by
the content management module

First, the NLU module produces an input frame for
the current event by analyzing the ASR hypotheses, the VUI output, and the dialogue state. Then, the
DM module examines the input frame, executes the dialogue policy, and updates the dialogue state.
The DM operates at two levels, with a master to manage the overall conversation and a collection of
miniskills to handle different types of conversation segments (discourse segments). Finally, the NLG
module uses the speech act and content selected by the DM module to build the response, which is
returned to the ASK and also stored as part of the conversation context in the DM module.

In terms of dialog policies,
Also, priority of individual policies.
In addition to the {\it recommendation policy} discussed in
\S\,\ref{chap1:ssec:recommendation_policy}, which constitutes the proactive
characteristic of the system, there are several other policies that are
essential for a socialbot.
{\it Context management policy} tracks necessary context information including
the dialog state and the user profile.
{\it Language understanding policy} enhances the SLU output with a certain level
of reasoning based on the context information.
Particularly, state-dependent SLU and implicit speech act.
{\it Language generation policy} selects proper speech acts and associated
arguments, and makes a plan of the response to be generated by the NLG module.
Multiple domains, domain-specific policies and policies that can be shared
across multiple domains.

In addition to the {\it recommendation policy} discussed in
\S\,\ref{chap1:ssec:recommendation_policy}, which constitutes the proactive
characteristic of the system, there are several other policies that are
essential for a socialbot.
{\it Context management policy} tracks necessary context information including
the dialog state and the user profile.
{\it Language understanding policy} enhances the SLU output with a certain level
of reasoning based on the context information.
Particularly, state-dependent SLU and implicit speech act.
{\it Language generation policy} selects proper speech acts and associated
arguments, and makes a plan of the response to be generated by the NLG module.
All these policies have been \dots, however, since socialbot is new, requires
further investigation in this area.

\noindent
{\bf SLU challenges}:
The wide coverage of domains, together with the great flexibility of human
language in causal conversations, leads to a long-tail distribution of user
utterances, which makes SLU significantly harder.
In particular, there is limited prior work on investigating the SLU for
socialbots, such as intents for informing topic and information source
preferences.
Moreover, understanding users' emotion states and opinions becomes more
crucial for socialbots compared with task-oriented systems due to the prevalence
of such utterances in socialbot conversations.

\noindent
{\bf DM challenges}:
Challenges for socialbot DM come from considerations on both system architecture
and dialog policy.
First, similar to open-domain dialog systems, the socialbot architecture needs
to be capable of accommodating a variety of domains.
Ideally, the architecture can isolate domain dependencies to avoid combinatorial
explosion in development and maintenance cost as the coverage of domains
increases, while allowing coherent transitions among domains during a
conversation.
Second, since the socialbot research is in the early stages, there are no prior
work on dialog policies to build upon for the involved domains.
The possible choices of domain taxonomy for socialbots may further complicate
the DM.
\hfang{While there are lots of things we can learn from previous work, e.g.,
dialog policy learning.}

\noindent
{\bf NLG challenges}:
Arguably, the NLG is often not the main focus in building or maintaining dialog
systems.
Most hand-crafted NLG modules, e.g., template-based or rule-based.
Nevertheless, NLG is critical in the development and system performance,
especially as other modules improves, the NLG becomes the short plate of a
dialog system (cask theory).
Considerations for conversational systems and socialbots.


